Can Agents Learn by Analogy? An Inferable Model for PAC Reinforcement Learning

Model-based reinforcement learning algorithms make decisions by building and utilizing a model of the environment. However, none of the existing algorithms attempts to infer the dynamics of any state-action pair from known state-action pairs before meeting it for sufficient times. We propose a new model-based method called Greedy Inference Model (GIM) that infers the unknown dynamics from known dynamics based on the internal spectral properties of the environment. In other words, GIM can "learn by analogy". We further introduce a new exploration strategy which ensures that the agent rapidly and evenly visits unknown state-action pairs. GIM is much more computationally efficient than state-of-the-art model-based algorithms, as the number of dynamic programming operations is independent of the environment size. Lower sample complexity could also be achieved under mild conditions compared against methods without inferring. Experimental results demonstrate the effectiveness and efficiency of GIM in a variety of real-world tasks.

==> 2.5_setup.tex <==
%!TEX root = 0_aamas20_tensor_rl_main.tex

%\section{Problem Setup}

%We concentrate on the problem of maximizing the total reward for a given MDP, and suppose we know the cardinality of $\states$ and $\actions$, denoted by $S$ and $A$ respectively. 
%
%To use spectral methods, we first represent the dynamics of the MDP with matrices defined as below. 

% Dynamic matrices can also be zipped \yc{which word?} into a tensor with dimension $S \times A \times (S+1)$, where every frontal fiber is corresponding to the whole dynamics of a state-action pair.




==> 2_prelim_old.tex <==
%!TEX root = 0_neurips19_tensor_rl_main.tex

\section{Preliminaries and Notations}
\label{sec:prelim}

We first introduce some notations and settings that we are going to use in this paper.

\begin{definition}[MDP]
An Markov decision process (MDP) is defined as a tuple $<\mathcal{S},\mathcal{A},P,R,\mu>$, where $S$ is the state space; $A$ is the action space; $P$ is the transition probability function with $P(s^\prime=s_j | s=s_i, a=a_k)$ representing the probability of transiting to state $s_j$ from state $s_i$ by taking action $a_k$; $R$ is the reward function with $R(s=s_i, a=a_k)$ recording the reward one can get by taking action $a_k$ in state $s_i$; $\mu$ is the initial state distribution. $P$ and $R$ together are called the dynamics of the MDP. We use $S$ and $A$ to denote the cardinalicy of $\mathcal{S}$ and $\mathcal{A}$.
\end{definition}

In this paper we focus on episodic, discrete-time, and fixed horizon MDPs with finite state and action spaces. A deterministic policy $\pi: S\rightarrow A$ defines what action an agent would take in a specific state. So by following a policy $\pi$, we can have a sequence of states, actions and rewards as $s_0, a_0, r_1, s_1, a_1, \cdots, r_H, s_H, a_H, r_{H+1}$.
 The value function of a policy $\pi$ for a given MDP $M$ with horizon $H$ (steps one can take in an episode) can be defined as the expected average reward
\begin{equation}
V^\pi_M = \mathbb{E}_{s_0 \sim \mu}[\frac{1}{H}\sum_{h=0}^{H-1} r(s_h, \pi(s_h))]
\end{equation}

The optimal policy $\pi^*$ is the policy that achieves the largest possible value $V^*_M$.

We will also use the following basic linear algebra notations.

Let $[n]:=\{1,2,\ldots,n\}$. 
For a vector $\myvector{v}$, denote the $i^{\tha}$ element as $v_i$. 
For a matrix $\mymatrix{M}$, denote the $i^{\tha}$ row as $\mymatrix{m}^i$, $j^{\tha}$  column as $\mymatrix{m}_j$, and $(i,j)^{\tha}$ element as $m_{ij}$.  
Denote  the first $r$ columns of matrix $\mymatrix{M}$ as $\mmCols{M}{r}$.
An $n$-order (number of dimensions, a.k.a. modes) tensor, denoted as $\mytensor{T}$, is a multi-dimensional array with $n$ dimensions.
For a 3-order tensor $\mytensor{T}$, its $(i,j,k)^{\tha}$ entry is denoted by $T_{ijk}$. 
%A tensor is called \textbf{cubical} if every mode is of the same size.  A cubical tensor is called \textbf{supersymmetric} (or simply refered as symmetric thereafter) if its elements remain constant under any permutation of the indices.

\textbf{Tensor product} is also known as outer product. 
For $\myvector{a} \in \R^m, \myvector{b} \in \R^n$ and $\myvector{c} \in \R^p$, $\myvector{a} \otimes \myvector{b} \otimes \myvector{c} $ is a $m \times n \times p$ sized 3-way tensor with $(i,j,k)^\tha$ entry being $a_ib_jc_k, \forall 1 \le i \le m, 1\le j \le n, 1\le k \le p$. 


% \textbf{Khatri-rao product}$\mymatrix{A}\! \odot\! \mymatrix{B}\!:=\!
% 	\begin{bmatrix}
% 	\vspace{-0.5em}a_{11} \mymatrix{b}_1 	&\hspace{-1em}\cdots&\hspace{-1em} 	a_{1p} \mymatrix{b}_p \\
% 	\vspace{-0.5em}\vdots 			    	&\hspace{-1em}\ddots&\hspace{-1em} 	\vdots \\
% 	a_{m1} \mymatrix{b}_1 	&\hspace{-1em}\cdots&\hspace{-1em} 	a_{mp} \mymatrix{b}_p 
% 	\vspace{-1em}
% 	\end{bmatrix}$, % ${\mathclap{\in \R^{mn\times p}}}$, 
% 	for $\mymatrix{A}$$\in$$\R^{m\times p}$, $\mymatrix{B}$$\in$$\R^{n\times p}$. 

%\textbf{Hadamard Product} of $\mymatrix{A}, \mymatrix{B} \in \R^{m\times n}$ is element-wise product.

\textbf{Tensor Operator Norm} The operator norm for tensor $\mytensor{T} \in \mathbb{R}^{d_1\times d_2 \times d_3}$ is defined as $\| \mytensor{T} \|_{\op} = \max\limits_{\myvector{\mu}_i \in \mathbb{R}^{d_i}\backslash{ \{\myvector{0}\}}, i=1,2,3} \frac{| \mytensor{T} (\myvector{\mu}_1, \myvector{\mu}_2,\myvector{\mu}_3) |}{\| \myvector{\mu}_1\| \cdot \|\myvector{\mu}_2\| \cdot \|\myvector{\mu}_3 \|}$.

\textbf{Matricization} is the process of reordering the elements of an $N$-way
tensor into a matrix.
The mode-$n$ matricization of
a tensor $\mytensor{T} \in \R^{I_1\times I_2\times \ldots \times I_N}$ is denoted by $\mytensor{T}_{(n)}$ and arranges the mode-$n$ fibers ~\cite{kolda2009tensor} to be the columns of the resulting matrix.
To be precise, the $(i_1, i_2,...,i_N)^\tha$ element of  the tensor maps to the $(i_n, j)^\tha$ element of the matrix, where $j=1+\sum_{k=1,k\neq n}^N (i_k-1)\prod_{m=1,m\neq n}^{k-1} I_m$.

\textbf{Fibers and Slices}

\textbf{CP Decomposition and Tensor Rank} \fh{TODO: Add.}

\textbf{Multi-linear Operation}


==> 3_model_v0.tex <==
%!TEX root = 0_neurips19_tensor_rl_main.tex
\section{Model}
\label{sec:model}

% \yc{
% \begin{enumerate}
% 	\item problem statement
% 	\item our definition of tensorial MDP
% 	\item high-level discussion about assumptions
% 	\item tensor methods (whitening, tensor decomposition, tensor completion)
% 	\item algorithm
% \end{enumerate}
% }

\subsection{Problem Setup}
In a reinforcement learning (RL) task, an agent usually does not know the dynamics (transition probability and reward function), sometimes even does not know the whole state space of the underlying MDP. What it can do is to interact with the MDP, i.e., to choose one action in every step. The general goal of RL algorithms is to learn the optimal policy for any given MDP with as few interactions as possible. A widely-used framework to measure the performance of RL algorithms is \textit{sample complexity of exploration} \cite{kakade2003sample}, or \textit{sample complexity} for short, which can be briefly defined by Definition~\ref{def:sc}. 

\begin{definition}[Sample complexity of exploration]
\label{def:sc}
For any $\epsilon>0$ and $0 < \delta < 1$, and at any step $0<h \leq H$, if the policy $\pi$ generated by an RL algorithm $L$ satisfys $V^*(s_h)-V^\pi(s_h) \leq \epsilon$, we say $L$ is near-optimal at step $h$. If with probability at least $1-\delta$, the total number of steps that $L$ is not near-optimal is upper bounded by a function $\zeta(\epsilon, \delta)$, then $\zeta$ is called the sample complexity of $L$.
\end{definition}

Intuitively, sample complexity measures the number of times in which the agent is not acting near-optimally. 
Lower sample complexity is always an important objective that RL algorithms want to achieve. 

In this paper, we propose a new model-based reinforcement learning method that considers the structure properties of MDPs. We first introduce a new representation of MDP as follows.

\begin{definition}[Tensorial Markov decision process, or TMDP]
	For an MDP $M$ denoted by tuple $<S, A, P, R, \mu>$, we can use a 3-order tensor $\tmdp \in \mathbb{R}^{|S| \times |S+1| \times |A|}$ to denote the dynamics of a MDP, where $\tmdp_{i,:,k}=[P(s_1|s_i,a_k), P(s_2|s_i,a_k), \cdots, P(s_{|S|}|s_i,a_k),R(s_i,a_k)]$. 
\end{definition}

So each frontal slice of $\tmdp$, denoted by $\tmdp_k, \forall 1 \leq k \leq |A|$ is a transition and reward matrix.

% By using tensors to represent the dynamics of MDPs, we can make good use of the structure of the MDPs and significantly accelerate the learning process. 
The definition of TMDP helps us make good use of the MDP structure, then we will show how it can significantly accelerate the learning process. To make our theoretical guarantees work well, we have two assumptions as follows. 

\begin{assumption}
\label{assum:lowrank}
	Assume every TMDP has a low rank sturcture. The upper bound of rank is known as $R$, which means the TMDP has the CP decomposition form
	$$
	\mathcal { M } = \sum _ { i = 1 } ^ { R } \lambda _ { i } \boldsymbol { a } _ { i } \otimes \boldsymbol { b } _ { i } \otimes \boldsymbol { c } _ { i }
	$$
	where $\boldsymbol{a}_i \in \mathbb{R}^{|S|}$, $\boldsymbol{b}_i \in \mathbb{R}^{|S|+1}$, and $\boldsymbol{c}_i \in \mathbb{R}^{|A|}$.
\end{assumption}

\begin{assumption}
\label{assum:linear_indep}
	Assume for any $i \neq i^\prime \leq R$, $\boldsymbol{a}_i$ and $\boldsymbol{a}_{i^\prime}$ are linearly independent. Similarly for $\boldsymbol{b}$ and $\boldsymbol{c}$. 
\end{assumption}

\yc{TODO: tensor completion assumptions}

Detailed analysis of the low-rankness is discussed in Section \ref{ana:lowrank}, where we will derive an upper bound of the TMDP's rank, so Assumption~\ref{assum:lowrank} is actually mild in practice. Assumption~\ref{assum:linear_indep} is natrual when the underlying MDP comes from a generative model. 

The key to many model-based algorithms like $E^3$\cite{kearns2002near} and $RMax$ \cite{brafman2003rmax} is to estimate the dynamics of MDPs through interactions. Once a state-action pair is visited by the agent for enough times, the estimations for the transition probabilities and average reward will be guaranteed to be nearly accurate with high probability. But it usually takes a long time and needs a huge number of samples to ``known'' all the state-action pairs. For example, it is proved \cite{kakade2003sample} that $\tilde{O}(\frac{|S|^2 |A| H^3}{\epsilon^3})$ actions of exploration are needed in $RMax$.

However, we can avoid estimating every single state-action pair, because the dynamics are not always totally in chaos. Think about \yc{an example here} 
Intuitively, an agent will learn much faster if it is smart enough to borrow knowledge from the experience with known states when interacting new states, or update its understanding to old states when knowing more states. Luckily, it is not impossible to make the agent this smart. Though tensor methods, we can easily estimate or recover the underlying dynamics of unknown state-action pairs collaboratively.

\subsection{Algorithm}

We can construct an observed TMDP by setting its entries with the following rules:
\begin{equation}
\label{eq:atmdp}
\forall (s_i,a_k), \atmdp_{i,j,k} = 
\left\{
\begin{aligned}
&\frac{n(s_j | s_i, a_k)}{n(s_i,a_k)} & & 1 \leq j \leq |S| \\
&\frac{R(s_i,a_k)}{n(s_i,a_k)} & & j = |S+1|
\end{aligned}
\right.
\end{equation}

where $n(s_i,a_k)$ is the total number of visits to state-action pair $(s_i,a_k)$, $n(s_j | s_i, a_k)$ the total number of transitions from $s_i$ to $s_j$ by taking action $a_k$ and $R(s_i,a_k)$ the total rewards for the transition $(s_i,a_j,s_k)$.

$\atmdp$ is an approximation of $\tmdp$, so we have $$\atmdp = \tmdp + \boldsymbol{\Phi}$$ where $\boldsymbol{\Phi}$ is a noise tensor. The more observations we have, the more accurate the approximation is. 

Our main goal is to recover $\tmdp$ based on $\atmdp$, i.e., return a tensor $\tmdp^*$ that is $\epsilon$-close to the original $\tmdp$. \yc{TODO: need a mathematical expression.}

\input{algos/tensor_rmax}

In reality, the structure of the noisy observations is not always the same. Sometimes we do not have adequate observations, or the irregular noise prevent the algorithm from getting accurate estimations of the dynamics. And occasionally the observations are very skew, and some states are difficute to reach. Thus, we reduce the noisy observations into two types and adopt two different tensor methods for the recovery of the tensor entries (MDP dynamics), \textit{tensor decomposition} and \textit{tensor completion}.

\paragraph{Tensor Decomposition}
\label{sec:tensor_docomp}
There are many tensor decomposition methods \cite{kolda2009tensor}. In this paper, we use CANDECOMP/PARAFAC (CP) decomposition \cite{kolda2009tensor}\cite{carroll1970analysis}, which is one of the most well-known decomposition model. in our setting, the basic idea of tensor decomposition is to find a CP decomposition with $R$ components which can compose a recovered tensor approximating the observations well. In Section~\ref{sec:analysis}, we prove that if the noise is bounded, then the recovered tensor can also approximate the original tensor well.

A TMDP $\mathcal{M} \in \mathbb{R}^{|S| \times |A| \times |S+1|}$ with rank $R$ satisfing Assumption~\ref{assum:lowrank} can be decomposed as
\begin{equation}
\tmdp = \sum _ { r = 1 } ^ R \lambda_r \boldsymbol{a}_r \otimes \boldsymbol{b}_r \otimes \boldsymbol{c}_r
\end{equation}
where $\boldsymbol{a}_r \in \mathbb{R}^{|S|}$, $\boldsymbol{b}_r \in \mathbb{R}^{|S|+1}$, and $\boldsymbol{c}_r \in \mathbb{R}^{|A|}$. 

Although tensor decomposition can be applied to tensors with asymmetric and non-orthogonal components, for computational guarantees, we need to whiten the original tensor into a well-structured one. The general idea is to find three matrices $W_A, W_B$ and $W_C$, such that

\begin{equation}
\wtmdp = \tmdp (W_A, W_B, W_C) = \sum_{r=1}^R w_r \boldsymbol{u}_r ^{\otimes3}
\end{equation}

where $\boldsymbol{u}_i \in \mathbb{R}^d$, and $\forall i \neq j, \boldsymbol{u}_i \boldsymbol{u}_j = 0$, i.e., the CP components of the whitened TMDP $\wtmdp$ are symmetric and orthogonal. Finding such $W_A, W_B$ and $W_C$ is not difficult by
just applying the symmetrization and whitening procedure introduced in Appendix~\ref{apd:symm} and Appendix~\ref{apd:whiten}, as long as the tensor satisfies Assumption~\ref{assum:linear_indep}.

% Then we can get 
% \begin{align}
% \atmdp (W_A, W_B, W_C) &= (\tmdp + \boldsymbol{\Phi})(W_A, W_B, W_C) 
% \end{align}

% Let $\mathcal{T} = \mathcal{M} (W_A, W_B, W_C)$, $\hat{\mathcal{T}} = \hat{\mathcal{M}} (W_A, W_B, W_C)$, and $\boldsymbol{\Psi} = \boldsymbol{\Phi} (W_A, W_B, W_C)$

% Thus let $\awtmdp = \atmdp (W_A, W_B, W_C)$ and $\boldsymbol{\Psi} = \boldsymbol{\Phi} (W_A, W_B, W_C)$, we have
% \begin{equation*}
% \awtmdp = \wtmdp + \boldsymbol{\Psi}
% \end{equation*}
% where $\wtmdp, \awtmdp, \boldsymbol{\Psi}$ are all $d \times d \times d$ tensors.

A recent paper \cite{li2018guaranteed} proposes a simultaneous tensor decomposition algorithm s-ASI, and provides a profounding bound for the allowed noise. So we will use s-ASI in our architecture.

% \begin{theorem}
% Assume $\awtmdp \in \mathbb{R}^{d\times d\times d}$ permits a CP decomposition form $\llbracket \boldsymbol{W}; \boldsymbol{U},\boldsymbol{U},\boldsymbol{U} \rrbracket + \boldsymbol{\Psi}$ where $\boldsymbol{U}$ is orthonormal.
% If for any $0 < \epsilon, \delta_0 < 1$ and any $1 \leq r \leq R$, the operator norm of the noise tensor $\boldsymbol{\Psi}$ is bounded by $\min \{ O( \frac{\epsilon}{\sqrt{R}}), O(\frac{\delta_0}{\sqrt{d}} )\}$, then s-ASI algorithm is able to return estimated $\boldsymbol{W}^*$ and $\boldsymbol{U}^*$, such that with probability $1-O(\delta_0)$, $|w_r - w_r^*| \leq \epsilon, \|\boldsymbol{u}_r - \boldsymbol{u}_r^*\| \leq \epsilon, \forall 1 \leq r \leq R$.
% \end{theorem}
% \yc{put in analysis section?}

\paragraph{Tensor Completion}
\label{sec:tensor_comp}
Tensor completion is widely used for estimating the missing values in partially observed tensor. For every task, define a binary mask tensor $\mytensor{P} \in \mathbb{R}^{|S| \times |A| \times |S+1|}$. $\mytensor{P}_{ijk}$ is set to 1 only when $|\atmdp_{ijk}-\tmdp_{ijk}| \leq \epsilon_0$ with probability at least $1-\delta_0$. Then the objective of tensor completion is to solve the optimization problem
\begin{align}
\begin{array} { l l } 
	\text{minimize}_{\mytensor{M}^*} &\| \mytensor{P} \odot (\mytensor{M}^* - \atmdp) \|_F^2 \\
	\text{subject to } &rank(\mytensor{M}^*) \leq R 
\end{array}
\end{align}
where $\odot$ denotes element-wise product.

\yc{TODO: paper and algorithm}



\input{algos/decomposition}

\input{algos/completion}





==> 3_model_v1.tex <==
%!TEX root = 0_neurips19_tensor_rl_main.tex
\section{Greedy-Walking Spectral Model}
\label{sec:model}

\yc{beta greedy walking, describe the algo}

In this section, we present a novel model-based reinforcement learning method that considers the structure properties of MDPs. 

\subsection{A New Representation of MDP}

To make use of the structure properties of MDPs, we first introduce a new representation of MDP.

\begin{definition}[Tensorial Markov decision process, or TMDP]
	For an MDP $M$ denoted by tuple $<S, A, P, R, \mu>$, we can use a 3-order tensor $\tmdp \in \mathbb{R}^{S \times A \times (S+1)}$ to denote the dynamics of a MDP, where $\tmdpv_{i,j,:}=[p(s_1|s_i,a_j), p(s_2|s_i,a_j), \cdots, p(s_{S}|s_i,a_j),r(s_i,a_j)]$. 
\end{definition}

So each lateral slice of $\tmdp$, denoted by $\tmdpm_{:j:}, \forall 1 \leq j \leq A$ is a transition and reward matrix for action $a_j$. The first $S$ frontal slices $\tmdpm_{::k} \text{ or } \tmdpm_k, \forall 1 \leq k \leq S$ are state-action transition matrices for the corresponding transit-in-state $s_k$. And the last frontal slice $\tmdpm_{::S+1}$ is the state-action reward matrix. For simplicity, we name the frontal slices as \textit{dynamic matrices}.





\subsection{Tensor-RMax Algorithm}

The key to many model-based algorithms like $E^3$\cite{kearns2002near} and RMax \cite{brafman2003rmax} is to estimate the dynamics of MDPs through interactions. Once a state-action pair is visited by the agent for enough times, the estimations for the transition probabilities and average reward will be guaranteed to be nearly accurate with high probability. 

RMax algorithm divides all states into two sets: ``known'' states $\mathcal{K}$ and ``unknwon'' states $\bar{\mathcal{K}}$. If a state-action pair is observed for sufficient times, say $m$, it becomes $m$-known to the agent. If for a specific state $s \in \mathcal{S}$, the pairs with all possible actions are all $m$-known, i.e., $\forall a \in \mathcal{A}, (s,a) $ is $m$-known, then $s \in \mathcal{K}$, otherwise $s \in \bar{\mathcal{K}}$. But it usually takes a long time and needs a huge number of samples to ``know'' all the state-action pairs.
 % For example, it is proved \cite{kakade2003sample} that $\tilde{O}(\frac{S^2 A H^3}{\epsilon^3})$ actions of exploration are needed in $RMax$.

However, we can avoid estimating every single state-action pair, because the dynamics are not always totally in chaos. In a maze or a gridworld, when the agent decides to go up, it will have the same probability of slipping to left or right. In a dialog system, the agent can use the same answer for a series of questions from the user. Such features can be described by the structure of a TMDP. If the TMDP has low-rank structure, or some of its slices are low-rank, then the underlying MDP is controled by some latent factors. Utilizing such latent factors through spectral methods can help us facilitate the learning process -- the agent would be able to borrow knowledge from the previous experience with known states to estimate the dynamics of unknown states.

\textbf{Construct Empirical TMDP}

TMDP models the dynamics of an MDP, but in practice, we can not get the true dynamics of the MDP. So we construct an empirical TMDP from observed data by setting its entries with the following rules:

\begin{equation}
\label{eq:atmdp}
\forall (s_i,a_k), \atmdps_{i,j,k} = 
\left\{
\begin{aligned}
&\frac{n(s_j | s_i, a_k)}{n(s_i,a_k)} & & 1 \leq j \leq |S| \\
&\frac{R(s_i,a_k)}{n(s_i,a_k)} & & j = |S+1|
\end{aligned}
\right.
\end{equation}

where $n(s_i,a_k)$ is the total number of visits to state-action pair $(s_i,a_k)$, $n(s_j | s_i, a_k)$ the total number of transitions from $s_i$ to $s_j$ by taking action $a_k$ and $R(s_i,a_k)$ the total rewards for the transition $(s_i,a_j,s_k)$.

$\atmdp$ is an approximation of $\tmdp$, so we have $$\atmdp = \tmdp + \noiset$$ where $\ \noiset$ is a noise tensor. The more observations we have, the more accurate the approximation is. 

Our main goal is to recover $\tmdp$ based on $\atmdp$, i.e., return a tensor $\rtmdp$ that is $\epsilon$-close to the original $\tmdp$, i.e., $\| \rtmdp - \tmdp \|_{\mathrm{max}} \leq \epsilon$.


% In reality, the structure of the noisy observations is not always the same. Sometimes we do not have adequate observations, or the irregular noise prevent the algorithm from getting accurate estimations of the dynamics. And occasionally the observations are very skew, and some states are difficute to reach. Thus, we reduce the noisy observations into two types and adopt two different tensor methods for the recovery of the tensor entries (MDP dynamics), \textit{tensor decomposition} and \textit{tensor completion}.

\textbf{Construct Known Mask}

Following the RMax algorithm, we also distinguish all state-action pairs as known and unknown with known threshold $m$.
And we can build a binary mask $\mask \in \mathbb{R}^{S \times A}$ by
\begin{equation}
	\masks_{i,j} = 
\left\{
\begin{aligned}
& 1 & & \text{if }(s_i,a_k) \text{ is known} \\
& 0 & & \text{otherwise}
\end{aligned}
\right.
\end{equation}

\textbf{Estimate Unknown Pairs via Matrix Completion}
\label{sec:completion}

%Matrix completion is widely used for estimating the missing values in partially observed matrices. For every task, define a binary mask tensor $\mytensor{P} \in \mathbb{R}^{|S| \times |A| \times |S+1|}$. $\mytensor{P}_{ijk}$ is set to 1 only when $|\atmdp_{ijk}-\tmdp_{ijk}| \leq \epsilon_0$ with probability at least $1-\delta_0$. Then the objective of tensor completion is to solve the optimization problem
Matrix completion is widely used for estimating the missing values in partially observed matrices. For every state-action transition matrix $\tmdpm_k$ with rank $r_k$, where $k \in [S+1]$, having sufficient number of known entries $\{ \tmdps_{ijk} | (s_i, a_j) \in \kset \}$, we are able to recover the other unknown (missing) entries by solving the optimization problem
\begin{align}
\begin{array} { l l } 
	\text{minimize}_{\rtmdpm_k} &\| \mask \odot (\rtmdpm_k - \tmdpm_k) \| \\
	\text{subject to } &rank(\rtmdpm_k) \leq r_k
\end{array}
\end{align}
where $\odot$ denotes element-wise product.


\input{algos/tensor_rmax}

The algorithm is described in Algorithm~\ref{alg:tensor_rmax}. $\fraction$ denotes the minimum rate of known state-action pairs among all state-action pairs. Completion operation will not be called until $\fraction SA$ state-action pairs become known. The main idea of \ourmod is to make at least $\fraction SA$ state-action pairs known and then perform matrix completion for every dynamic matrix. Different with balanced wandering, which is used in both $\text{E}^3$ and RMax algorithm to let the exploration as fair as possible, we design a $\beta$-greedy walking strategy for action slection in unknown states.

\textbf{$\boldsymbol{\beta}$-greedy Walking}

We first define the concept of $\fraction$-known. A state $s$ is $\fraction$-known if there exist $\fraction A$ distinct actions such that $(s,a)$ is known or $m$-known. Then we can design a greedy walking strategy as: if the current state is $\fraction$-known, then randomly select actions until a non-$\fraction$-known state is encountered; if the current state is not $\fraction$-known, then choose an action $a = \argmax_a\{ n(s,a) | (s,a) \text{ is unknown} \}$. Notice that when the maximum is not unique, a random selection among all maximum values should be executed. Then, $\beta$-greedy walking strategy is to choose actions randomly with probability $\beta$, and run greedy walking with probability $1-\beta$, when the current state is not $\fraction$-known.


% \input{algos/decomposition}

% \input{algos/completion}





==> 4_analysis_1.tex <==
%!TEX root = 0_neurips19_tensor_rl_main.tex
\section{Analysis}
\label{sec:analysis}



% \subsection{Low-rankness of TMDP}
% \label{ana:lowrank}

% \yc{a real world example about low-rank transition matrix}
% \begin{figure}[!htb]
%     \center{\includegraphics[width=0.2\textwidth]
%     {\fighome/example.png}}
%     \caption{A simple example of a grid world.}
%     \label{fig:example}
% \end{figure}

% Consider the simplest gridworld example shown in Figure~\ref{fig:example}, where each of the grid is a state. The agent can take actions "up", "down", "left", and "right" from every state, and "slip" with probability 0.4, which means when it takes action "right", it may go right with probability 0.6, but go up or down each with probability 0.2.
% Then the transition matrix under action "right" is

% \begin{equation*}
% \left[
% \begin{matrix} 
% 0.2 & 0.6 & 0.2 & 0   \\
% 0 	& 0.8 & 0	& 0.2 \\ 
% 0.2 & 0	  & 0.2 & 0.6 \\
% 0	& 0.2 & 0	& 0.8
% \end{matrix}
% \right]
% \end{equation*}

% \subsection{PAC Bound of Tensor-RMax}
% \label{ana:sc}
In this section, we will analyze the sample complexity of \ourmod. Although we consider the worst case for the derivation of upper bound, the actual samples we need can be much less than this bound in reality.

Our analysis makes these assumptions: 

\begin{enumerate}
\label{assumptions}
	\item For the object MDP, there is a knwon diameter $D$, such that any state $s^\prime$ is reachable from any state $s$ in at most $D$ steps on average.
	\item The horizon $H \gg D$.
	\item The condition number and the rank of every dynamic matrix are upper bounded by $\kappa$ and $r$ respectively, which are known to the model.
	\item All dynamic matrices are $(\mu_0, \mu_1)$-incoherent, and $\mu_0, \mu_1$ are known to the model.
	\item The distribution of the estimation noise is sub-Gaussian with mean $\mathbb{E}(\noises_{ijk}) = 0$. And the estimation noises for different state-action pairs are independent.
\end{enumerate}

% (1) For the object MDP, there is a knwon diameter $D$, such that any state $s^\prime$ is reachable from any state $s$ in at most $D$ steps on average. (2) For any known state-action pair $(s,a)$, define the estimation noise of any $s^\prime \in \mathcal{S}$ as $\eta = \ |p(s^\prime | s, a) -  \hat{p}(s^\prime | s, a)|$. Assume the distribution of $s^\prime$ is sub-Gaussian with parameter $C$. So we have $\mathbb{P}(| \eta - \mathbb{E}[\eta|s,a] | \geq \lambda) \leq 2 \mathrm{exp}(-C\lambda^2)$.

The first assumption about the diameter is very commonly used in reinforcement learning theories. It is first introduced by Jaksch et al. in \cite{jaksch2010near}. This is to ensure that on average every state is reachable no matter what the current state is. The second assumption is also very mild because the horizon is often set large, and it makes sure that in each episode, all states should be met. The third assumption helps us set the best known threshold. It is not hard to know the upper bound for a specific kind of task. 
% The second assumption is also mild that the noise has strong tail decay property, because the estimation is evenly taken for every state.

Without loss of generality, suppose $S \geq A$, then we have Theorem~\ref{thm:main}.

\begin{theorem}[Sample Complexity of \ourmod] 
\label{thm:main}
	Given an MDP $M$ with horizon $H$, and the corresponding TMDP $\tmdp$, for any $0<\epsilon<1$, $3/A^3 \leq \delta < 1$, and with completion fraction $\fraction \geq \mathcal{O}(\frac{1}{\sqrt{SA}}\kappa^2 \max\{ \mu_0 r \sqrt{\frac{S}{A}} \log A, \mu_0^2 r^2 \frac{S}{A} \kappa^4, \mu_1^2 r^2 \frac{S}{A} \kappa^4 \})$, \text{\ourmod } algorithm \ref{alg:tensor_rmax} can produce a policy $\hat{\pi}$, which satisfys $V^{\hat{\pi}}_M \geq V^*_M - \epsilon$ for all but 
	$$
	\max\{ \mathcal{O}(\frac{\fraction S^2 A H^2}{(1-\beta)\epsilon^3} \log \frac{1}{\delta} \log \frac{\fraction SA}{\delta}), \mathcal{O}(\frac{\kappa^4 r (S+1)^2 \sqrt{S A^3} H^2}{\fraction (1-\beta) \epsilon^3} \log \frac{1}{\delta} \log^2 \fraction SA) \}
	$$ 
	episodes, with probability at least $1-\delta$.
\end{theorem}

% \textbf{Remark.} TBD.

% \textbf{Proof Sketch.} We first prove in Lemma~\ref{lem:sc_m} that with known threshold $m$, $\mathcal{O}(\frac{m\rho SA}{\epsilon} \mathrm{ln}\frac{1}{\delta})$ non-optimal episodes are needed. Then we find the minimum feasible value of $m$ such that the estimation of known state-action pairs is accurate enough.

Let $m$ be the number of visits needed to make a state-action pair known, and we assume the following condition holds for $m$:
\begin{condition}
\label{cond:m}
	The known threshold $m$ is chosen such that the optimal policy $\hat{\pi}$ for $\hat{M}_\kset$ satisfys 
	\begin{equation}
	\label{eq:m_cond_k}
		V^{\hat{\pi}}_{M_\kset} \geq V^{*}_{M_\kset} - \epsilon,
	\end{equation}
	and after completion, it satisfys
	\begin{equation}
	\label{eq:m_cond_all}
		V^{\hat{\pi}}_{M} \geq V^{*}_{M} - \epsilon.
	\end{equation}
\end{condition}



Then with the parameter $m$, we can express the sample complexity as

\begin{lemma}[Sample Complexity in terms of $m$]
\label{lem:sc_m}
	Let $M$ be an MDP with fixed horizon $H$. If $\tilde{\pi}$ is the policy computed by \ourmod, then for any starting state $s_0$, with probability at least $1-2\delta$, we have $V_M^{\tilde{\pi}} \geq V_M^* - 2 \epsilon$ for all but $\mathcal{O}(\frac{m\rho SA}{(1-\beta)\epsilon} \log \frac{1}{\delta})$
\end{lemma}
% \fh{Need to compare with Rmax and E${}^3$.}
\textbf{Remark.} For Rmax algorithm, the sample complexity is $\mathcal{O}(\frac{mSA}{\epsilon} \log \frac{1}{\delta})$. $\beta$ is the probability of randomly selecting action, which can be set by hand. So the less entries required for completion, the less non-optimal episodes in the learning process.

% \textbf{Proof Sketch.} TBD 

Lemma~\ref{lem:pertur_bound} is also needed to prove the main theorem. 

\begin{lemma}[Perturbation Bound of Tensor Completion]
\label{lem:pertur_bound}
	Let $\tmdp \in \mathbb{R}^{S \times (S+1) \times A}$ be the groud truth TMDP for a specific RL task, and $\atmdp \in \mathbb{R}^{S \times (S+1) \times A}$ be the empirical TMDP for the same task. Let $\noiset$ be the noise tensor, so $\atmdp = \tmdp + \noiset$.
	If the entries of $\noisem_k$ are i.i.d. random variables with zero mean and sub-Gaussian tails with variance proxy $\sigma^2$, then with probability at least $1-1/A^3$ the result TMDP $\rtmdp$ returned by the function \textit{MatrixCompletion}($\atmdp$) \ref{alg:tensor_rmax} satisfys 
	$$
	\| \tmdp - \rtmdp \|_{\text{max}} \leq \mathcal{O} \Big( \frac{\kappa^2 \sqrt{r} \log \fraction SA}{\fraction \sqrt[4]{A^5 S}} \sigma \Big),
	$$
	provided that
	$$
	\fraction \geq \Omega(\frac{1}{\sqrt{SA}}\kappa^2 \max\{ \mu_0 r \sqrt{\frac{S}{A}} \log A, \mu_0^2 r^2 \frac{S}{A} \kappa^4, \mu_1^2 r^2 \frac{S}{A} \kappa^4 \} ),
	$$
	where $\fraction$ is the fraction of observed entries, $\kappa$ and $r$ are respectively the supremum of the condition number and the rank of all dynamic matrices.
\end{lemma}



















==> algos/completion.tex <==
%!TEX root = ../0_neurips19_tensor_rl_main.tex
% \begin{algorithm}
% \caption{Tensor-RMax (completion)}\label{alg:tr_comp}
% \begin{algorithmic}[1]
% \STATE 1
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
\DontPrintSemicolon
\caption{Tensor Completion}\label{alg:comp}
  \Parameter{Least number of known entries $\eta$}
  \Fn{\Ma{$n(s_:,a_:)$}}{
  	$\hat{\eta} \leftarrow | \{(s,a) | n(s,a) \geq m_0\} | $ \;
  	\eIf{$\hat{\eta} \geq \eta$}{
	   \KwRet true\;
	   }{
	   \KwRet false\;
	}
  }
  \Fn{\Re{$\atmdp$}}{
  	\textit{Symmetrization:}\;
  	\textit{Whitening:}\;
  	\textit{Decomposition:}\;
  	\KwRet $\btmdp$
  }
\end{algorithm}

==> algos/decomposition.tex <==
%!TEX root = ../0_neurips19_tensor_rl_main.tex

% \begin{algorithm}
% \caption{Tensor Decomposition}\label{alg:decom}
% \begin{algorithmic}[H]
% \STATE
% \STATE \textbf{Function} \textit{Mature} ($\atmdp$):
% \begin{ALC@g}
% 	\STATE TEST
% \end{ALC@g}

% \STATE \textbf{Function} \textit{Recover} ($\atmdp$):
% \begin{ALC@g}
% 	\STATE TEST
% \end{ALC@g}
% \end{algorithmic}
% \end{algorithm}

  
\begin{algorithm}
\DontPrintSemicolon
\caption{Tensor Decomposition}\label{alg:decom}
  \Parameter{Known threshold of tensor decomposition $m$}
  \Fn{\Ma{$n(s_:,a_:)$}}{
  	\eIf{$n(s_i,a_k) \geq m, \forall i,k$}{
	   \KwRet true\;
	   }{
	   \KwRet false\;
	}
  }
  \Fn{\Re{$\atmdp$}}{
  	\textit{Symmetrization:}\;
  	\textit{Whitening:}\;
  	\textit{Decomposition:}\;
  	\KwRet $\btmdp$
  }
\end{algorithm}

==> algos/tensor_rmax.tex <==
%!TEX root = ../0_neurips19_tensor_rl_main.tex
% \begin{algorithm}
% \caption{Tensor-RMax}\label{alg:tensor_rmax}
% \begin{algorithmic}[1]
% \REQUIRE Known threshold of RMax $m_0$
% \ENSURE Near-optimal policy $\hat{\pi}$
% \STATE Initialize $\atmdp \in \mathbb{R}^{|S| \times |S+1| \times |A|}$ by Equation \yc{TODO}
% \STATE Set $n(s_i,a_k)=0$, $n(s_j|s_i,a_k)=0$, $r(s_i,a_k)=0$, $\forall i,j,k$
% \FOR {episode $t=1$ to $T$}
% 	\STATE $s_1$ $\leftarrow$ initial state
% 	\FOR {step $h=1$ to $H$}
% 		\IF {$\sum_k n(s_h,a_k) \geq m_0 \times |A|$}
% 			\STATE Choose $a_h$ with current optimal policy $\hat{\pi}$
% 		\ELSE
% 			\STATE Randomly choose $a_h$ from $\{ a | n(s_h,a) < m_0 \}$
% 			\STATE Execute $a_h$, and get next state $s_{h+1}$, reward $r_{h+1}$
% 			\STATE $n(s_h,a_h) \leftarrow n(s_h,a_h) + 1$
% 			\STATE $n(s_{h+1}|s_h,a_h) \leftarrow n(s_{h+1}|s_h,a_h) + 1$
% 			\STATE $r(s_h,a_h) \leftarrow r(s_h,a_h) + 1$
% 			% \STATE Update: 
% 			% 		\begin{align*}
% 			% 			&n(s_h,a_h) \leftarrow n(s_h,a_h) + 1 \\
% 			% 			&n(s_{h+1}|s_h,a_h) \leftarrow n(s_{h+1}|s_h,a_h) + 1 \\
% 			% 			&r(s_h,a_h) \leftarrow r(s_h,a_h) + 1 \\
% 			% 		\end{align*}
% 			\STATE Update $\atmdp$ by Equation~\ref{eq:atmdp}
% 			\IF {\textit{Mature}($\atmdp$)}
% 				\STATE $\btmdp \leftarrow$ \textit{Recover}($\atmdp$)
% 				\STATE Set $n(s_i,a_k)=m_0, \forall i,k$
% 			\ENDIF
% 		\ENDIF
% 	\ENDFOR
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}


\begin{algorithm}[!htbp]
\DontPrintSemicolon
\caption{Tensor-RMax}
\label{alg:tensor_rmax}
  \Input{Epsidoe number $T$; horizon $H$; error tolerance $\epsilon$; known threshold $m$; completion fraction threshold $\fraction$; walking parameter $\beta$; upper bound of rank $r$}
  \Output{Near-optimal policy $\tilde{\pi}$ such that $V^{\tilde{\pi}} \geq V^* - \epsilon$}
  Initialize $\atmdp \in \mathbb{R}^{S \times A \times S+1}$ as all zeros \;
  $\forall i,j,k$, set $n(s_i,a_k)=0$, $n(s_j|s_i,a_k)=0$, $r(s_i,a_k)=0$ \;
  \For{episode $t\leftarrow 1$ \KwTo $T$}{
  	$s_1 \leftarrow$ initial state \;
  	\For{step $h\leftarrow 1$ \KwTo $H$}{
  		% \eIf{$\forall a, (s_h,a)$ is $m$-known}{
  		% 	Choose $a_h$ with current optimal policy $\hat{\pi}$ \;
  		% }{
  		% 	Choose $a_h$ using $\beta$-greedy walking strategy \;
  		% 	Execute $a_h$, and get next state $s_{h+1}$, reward $r_{h+1}$ \;
  		% 	\Up{$s_h,a_h,r_{h+1},s_{h+1},\atmdp$} \;
  		% 	\If{total number of known state-action pairs $ \geq \fraction S A$}{
  		% 		$\rtmdp \leftarrow$ \Re{$\atmdp$} \;
  		% 	}
  		% }
      \eIf{total number of known state-action pairs $ < \fraction S A$}{
        Choose $a_h$ using $\beta$-greedy walking strategy \;
        Execute $a_h$, and get next state $s_{h+1}$, reward $r_{h+1}$ \;
        \Up{$s_h,a_h,r_{h+1},s_{h+1},\atmdp$} \;
        \If{total number of known state-action pairs $ \geq \fraction S A$}{
          $\rtmdp \leftarrow$ \Re{$\atmdp$} \;
        }
      }{
        Choose $a_h$ with optimal policy $\tilde{\pi}$ \;
      }
  	}
  }
  \Fn{\Up{$s,a,r,s^\prime,\atmdp$}}{
  	$n(s,a) \leftarrow n(s,a) + 1$ \;
  	$n(s^\prime|s,a) \leftarrow n(s^\prime|s,a) + 1$ \;
  	$r(s,a) \leftarrow r(s,a) + 1$ \;
  	Update $\atmdp$ by Equation~\ref{eq:atmdp} \;
  }
  \Fn{\Re{$\atmdp$}}{
    Initialize $\rtmdp \in \mathbb{R}^{S \times A \times S+1}$\;
    \For{$k\leftarrow 1$ \KwTo $S+1$}{
      $\rtmdpm_k \leftarrow$ \MC{$\tmdpm_k, r$} \;
    }
    Set all state-action pairs as known \;
    Compute the optimal policy $\tilde{\pi}$ \;
  }
\end{algorithm}







==> figure_th_avg.tex <==
%!TEX root = 0_aaai20_tensor_rl_main.tex
\begin{figure*}[h]
\centering
	\begin{subfigure}[t]{0.3\textwidth}
		% \includegraphics[trim=10 10 50 50, clip,width=\textwidth]{\figPhome/gc_tf_layers.eps}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/avg/lowrank_S=20_A=10_r=2_runs=3.tex}	  	
		% \vspace{-1.25em}
	  	\caption{rank=2}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.3\textwidth}
		% \includegraphics[trim=10 10 50 50, clip,width=\textwidth]{\figPhome/gc_tnb_layers.eps} 
		\centering
		%\vspace{-1em}
		\input{\fighome/avg/lowrank_S=20_A=10_r=4_runs=3.tex}
		% \vspace{-1.25em}
	  	\caption{rank=4}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.3\textwidth}
		% \includegraphics[trim=10 10 50 50, clip,width=\textwidth]{\figPhome/gc_theta_layers.eps}
		\centering
		\input{\fighome/avg/lowrank_S=20_A=10_r=6_runs=3.tex}	  
		% \vspace{-1.25em}	
	  	\caption{rank=6}
	\end{subfigure}
	% \vspace{-0.6em}
  	\caption{Comparison of average reward of RMax and \ourmod on synthetic task with 20 states, 10 actions and different ranks. } 
	\label{fig:th_avg}
\end{figure*}


\begin{figure*}[h]
\centering
\vspace{-1em}
	\begin{subfigure}[t]{0.3\textwidth}
		% \includegraphics[trim=10 10 50 50, clip,width=\textwidth]{\figPhome/gc_tf_layers.eps}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/avg/gridworld_h=3_w=2_runs=10.tex}	  	
		% \vspace{-1.25em}
	  	\caption{3$\times$2 grid world}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.3\textwidth}
		% \includegraphics[trim=10 10 50 50, clip,width=\textwidth]{\figPhome/gc_tnb_layers.eps} 
		\centering
		%\vspace{-1em}
		\input{\fighome/avg/gridworld_h=3_w=3_runs=10.tex}
		% \vspace{-1.25em}
	  	\caption{3$\times$3 grid world}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.3\textwidth}
		% \includegraphics[trim=10 10 50 50, clip,width=\textwidth]{\figPhome/gc_theta_layers.eps}
		\centering
		\input{\fighome/avg/gridworld_h=4_w=4_runs=10.tex}	  
		% \vspace{-1.25em}	
	  	\caption{4$\times$4 grid world}
	\end{subfigure}
	% \vspace{-0.6em}
  	\caption{Comparison of average reward of RMax and \ourmod on grid world tasks with different sizes.} 
	\label{fig:th_avg_grid}
\end{figure*}

==> figure_th_compare_lowrank.tex <==
%!TEX root = 0_aaai20_tensor_rl_main.tex
\begin{figure}[!htbp]
\centering
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/avg/lowrank_S=20_A=10_r=2_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\avgrew}
	  	\label{sfig:com_avg_rank2}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/avg/lowrank_S=20_A=10_r=4_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\avgrew}
	  	\label{sfig:com_avg_rank4}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/avg/lowrank_S=20_A=10_r=6_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\avgrew}
	  	\label{sfig:com_avg_rank6}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/avg/lowrank_S=20_A=10_r=8_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\avgrew}
	  	\label{sfig:com_avg_rank8}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/avg/lowrank_S=20_A=10_r=10_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\avgrew}
	  	\label{sfig:com_avg_rank10}
	\end{subfigure}
  	\caption{Comparison of \avgrew} 
	\label{fig:th_compare_avg}
\end{figure}

\begin{figure}[!htbp]
\centering
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/times/lowrank_S=20_A=10_r=2_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\pavgrew}
	  	\label{sfig:com_times_rank2}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/times/lowrank_S=20_A=10_r=4_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\pavgrew}
	  	\label{sfig:com_times_rank4}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/times/lowrank_S=20_A=10_r=6_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\pavgrew}
	  	\label{sfig:com_times_rank6}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/times/lowrank_S=20_A=10_r=8_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\pavgrew}
	  	\label{sfig:com_times_rank8}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/times/lowrank_S=20_A=10_r=10_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\pavgrew}
	  	\label{sfig:com_times_rank10}
	\end{subfigure}

  	\caption{Comparison of \numepi} 
	\label{fig:th_compare_times}
\end{figure}

\begin{figure}[!htbp]
\centering
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/pavg/lowrank_S=20_A=10_r=2_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\pavgrew}
	  	\label{sfig:com_pavg_rank2}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/pavg/lowrank_S=20_A=10_r=4_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\pavgrew}
	  	\label{sfig:com_pavg_rank4}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/pavg/lowrank_S=20_A=10_r=6_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\pavgrew}
	  	\label{sfig:com_pavg_rank6}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/pavg/lowrank_S=20_A=10_r=8_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\pavgrew}
	  	\label{sfig:com_pavg_rank8}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.18\columnwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/appendix/pavg/lowrank_S=20_A=10_r=10_runs=20.tex}	  	
		% \vspace{-1.25em}
	  	% \caption{\pavgrew}
	  	\label{sfig:com_pavg_rank10}
	\end{subfigure}

  	\caption{Comparison of \pavgrew} 
	\label{fig:th_compare_pavg}
\end{figure}



==> figure_th_pavg.tex <==
%!TEX root = 0_aaai20_tensor_rl_main.tex
\begin{figure*}[h]
\centering
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/pavg/lowrank_S=20_A=10_r=2_runs=3.tex}	  	
		% \vspace{-1.25em}
	  	\caption{rank=2}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		%\vspace{-1em}
		\input{\fighome/pavg/lowrank_S=20_A=10_r=4_runs=3.tex}
		% \vspace{-1.25em}
	  	\caption{rank=4}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\input{\fighome/pavg/lowrank_S=20_A=10_r=6_runs=3.tex}	  
		% \vspace{-1.25em}	
	  	\caption{rank=6}
	\end{subfigure}
	% \vspace{-0.6em}
  	\caption{Comparison of average reward after exploration of RMax and \ourmod on synthetic dataset with 20 states, 10 actions and different ranks. $^\dag$} 
	\label{fig:th_pavg}
\end{figure*}

\begin{figure*}[h]
\centering
% \vspace{-1.25em}
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/pavg/gridworld_h=3_w=2_runs=10.tex}	  	
		% \vspace{-1.25em}
	  	\caption{3$\times$2 grid world}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		%\vspace{-1em}
		\input{\fighome/pavg/gridworld_h=3_w=3_runs=10.tex}
		% \vspace{-1.25em}
	  	\caption{3$\times$3 grid world}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\input{\fighome/pavg/gridworld_h=4_w=4_runs=10.tex}	  
		% \vspace{-1.25em}	
	  	\caption{4$\times$4 grid world}
	\end{subfigure}
	% \vspace{-0.6em}
  	\caption{Comparison of non-optimal episodes of RMax and \ourmod on grid world tasks with different sizes. $^\dag$ \\
  	\rule{0in}{1.2em}$^\dag$\scriptsize Because of the randomness of the MDP, RMax agent or \ourmod agent sometimes get rewards higher than the optimal agent.} 
	\label{fig:th_pavg_grid}
\end{figure*}

% \footnotetext[1]{Because of the randomness of the MDP, RMax agent or \ourmod agent sometimes get rewards higher than the optimal agent.}

==> figure_th_times.tex <==
%!TEX root = 0_aaai20_tensor_rl_main.tex
\begin{figure*}[h]
\centering
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/times/lowrank_S=20_A=10_r=2_runs=3.tex}	  	
		% \vspace{-1.25em}
	  	\caption{rank=2}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		%\vspace{-1em}
		\input{\fighome/times/lowrank_S=20_A=10_r=4_runs=3.tex}
		% \vspace{-1.25em}
	  	\caption{rank=4}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\input{\fighome/times/lowrank_S=20_A=10_r=6_runs=3.tex}	  
		% \vspace{-1.25em}	
	  	\caption{rank=6}
	\end{subfigure}
	% \vspace{-0.6em}
  	\caption{Comparison of non-optimal episodes of RMax and \ourmod on synthetic dataset with 20 states, 10 actions and different ranks. } 
	\label{fig:times}
\end{figure*}


\begin{figure*}[h]
\centering
% \vspace{-1.25em}
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		% \vspace{-0.25em}
		\input{\fighome/times/gridworld_h=3_w=2_runs=10.tex}	  	
		% \vspace{-1.25em}
	  	\caption{3$\times$2 grid world}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		%\vspace{-1em}
		\input{\fighome/times/gridworld_h=3_w=3_runs=10.tex}
		% \vspace{-1.25em}
	  	\caption{3$\times$3 grid world}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\input{\fighome/times/gridworld_h=4_w=4_runs=10.tex}	  
		% \vspace{-1.25em}	
	  	\caption{4$\times$4 grid world}
	\end{subfigure}
	% \vspace{-0.6em}
  	\caption{Comparison of non-optimal episodes of RMax and \ourmod on grid world tasks with different sizes.} 
	\label{fig:times_grid}
\end{figure*}

==> figures/mus/admu_rew_th40_mu0.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}[scale=0.3]

\definecolor{color0}{rgb}{0.462745098039216,0.654901960784314,0.490196078431373}
\definecolor{color1}{rgb}{0.4,0.470588235294118,0.67843137254902}

\begin{axis}[
legend cell align={left},
legend style={at={(0.03,0.03)}, anchor=south west, draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={Lowrank S=20 A=10 R=2 th=40},
x grid style={white!69.01960784313725!black},
xlabel={Incoherence Parameter},
xmajorgrids,
xmin=2.1857453316484, xmax=5.15548044390492,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Average Reward},
ymajorgrids,
ymin=0.517004943176365, ymax=1.01920940004133,
ytick style={color=black}
]
\addplot [only marks, draw=color0, fill=color0, colormap/viridis]
table{%
x                      y
2.33853895124789 0.944116814584662
2.35530534342027 0.967471069285448
2.40889192192327 0.946594039553198
2.43124458114077 0.961592638526264
2.64439927751083 0.937705853407171
2.8124648649877 0.954359913077758
2.81315941323757 0.956989083333359
2.8178491799041 0.628507982065746
2.85655348991692 0.897997873577612
2.85973443261204 0.952344078969386
2.86054013080652 0.945225389060984
2.88612360370583 0.901930281008516
2.89687947660398 0.951598264643036
2.90742783600007 0.952122420424514
2.91119709283638 0.866353106965441
2.92510490600092 0.983107749110406
2.92736379889279 0.974493411824409
2.93904242566529 0.98574204188208
2.94642166943524 0.858873456295494
2.95069010153344 0.607886205581111
2.95347825235203 0.899104132547077
2.96739269729362 0.960812207170544
2.97754291542565 0.58246623336033
2.98248479730667 0.838045108831744
2.99354777637743 0.952271207676458
3.00373746283297 0.667083771083648
3.06870009706479 0.948036688522127
3.09140083477183 0.961449891340915
3.09901107146927 0.942768756120005
3.1015462243679 0.9387916721792
3.11119400487178 0.838574622680684
3.11554845300908 0.942637537805773
3.11988316682247 0.955634407396855
3.12949999390849 0.813827127949491
3.14290945267774 0.955984384064372
3.14617608555766 0.970794966680039
3.17121235011721 0.642257966565738
3.17432549884301 0.930404644668184
3.22412135560557 0.834940868256853
3.22670676032307 0.979207014444986
3.22823762583094 0.9256790950657
3.22894596736215 0.934113753283207
3.22899816671053 0.920463615857986
3.24084712466588 0.939770677229503
3.24476134146831 0.850604274175127
3.24869274451924 0.626698855014324
3.26363109782957 0.908601336086781
3.26494280062718 0.966409382961427
3.27217664416401 0.965432151990657
3.27551413379116 0.848019844256498
3.27577178037818 0.967712763110733
3.2877568510935 0.741105965614382
3.29033090734629 0.784429816627742
3.2954417398048 0.931332970713218
3.31450622284833 0.972932048733155
3.32225913157062 0.982461558475317
3.32795735306142 0.925025777006423
3.32839473401103 0.961393289725869
3.33040474346732 0.917699682245254
3.33265418839896 0.886937534735762
3.33611311101724 0.860787048486992
3.34087237065333 0.967525056705756
3.35172877768159 0.89045205560879
3.35328914139082 0.881645217907425
3.39386116368422 0.965393312331509
3.39742533005062 0.973489235071986
3.40363407071089 0.796760146031483
3.40808488449723 0.845244388859193
3.41076104807395 0.908284375076073
3.41094394245119 0.958584815451437
3.41379024164085 0.962333546711216
3.42384797282245 0.976223362583378
3.42434582094298 0.948285502147399
3.43156517019436 0.932067268194557
3.43236603001016 0.902038170604955
3.43328643641677 0.901899472977276
3.44045231754726 0.949489465128746
3.44226737011648 0.9432444098366
3.44300952055236 0.979711682999047
3.44589523500906 0.932027658347507
3.44906410842006 0.965062010875084
3.45690151265941 0.966827165964829
3.47583248595385 0.719373404775628
3.47615234576982 0.905749330662503
3.48658939263647 0.674673456194466
3.48794276718236 0.929561277718458
3.50237823274565 0.894981503812532
3.50359405673934 0.908579533924475
3.53124611556688 0.979126629183511
3.54818974185777 0.959680752214066
3.58257325636424 0.966752764632305
3.60141451592631 0.960415248990536
3.6142109249443 0.942601994079041
3.61793367487007 0.681718955762535
3.62887539099232 0.918439704343155
3.64167752793328 0.547949301605292
3.64909113189349 0.934399763499205
3.66826146816848 0.955535415943164
3.71270603855035 0.968221746344972
3.7228756077762 0.55940433252471
3.7267930173775 0.971824114492466
3.73105877506751 0.876005722153962
3.76536145488467 0.92639179839568
3.78042999910134 0.924149678818448
3.79337096187177 0.911215163141547
3.79537903607238 0.940473303533892
3.85076838354008 0.941939880125672
3.88420179484695 0.753795546506044
3.9149293206751 0.779541560411298
3.91513139142539 0.899436111035418
3.9170808528953 0.972356815264247
3.97055345276468 0.685681756928028
4.0441461021308 0.986466960386943
4.11521533810174 0.978969976030392
4.12134504248109 0.959776904427451
4.3327422865046 0.959454947386707
4.38313514401762 0.969369925797597
4.40296794743456 0.950292633633619
4.81962996095038 0.818337520395251
5.00268682430542 0.980306670903351
};
\addlegendentry{RMax}
\addplot [only marks, draw=color1, fill=color1, colormap/viridis]
table{%
x                      y
2.33853895124789 0.976951817402363
2.35530534342027 0.978939809342585
2.40889192192327 0.984888595740123
2.43124458114077 0.973535803578934
2.64439927751083 0.980225502964051
2.8124648649877 0.984526761545926
2.81315941323757 0.984846942352842
2.8178491799041 0.984175713096747
2.85655348991692 0.983559880263691
2.85973443261204 0.986482548237323
2.86054013080652 0.981182619522777
2.88612360370583 0.961963577801265
2.89687947660398 0.98691353640538
2.90742783600007 0.981494471564227
2.91119709283638 0.986180401795894
2.92510490600092 0.984664588046099
2.92736379889279 0.967992191849219
2.94642166943524 0.979853479081902
2.95069010153344 0.9852557378269
2.95347825235203 0.983164291299059
2.96739269729362 0.987102477787357
2.97754291542565 0.973665247245119
2.98248479730667 0.981792033406558
2.99354777637743 0.984284458016046
3.00373746283297 0.975837386627959
3.06870009706479 0.974905991589027
3.09140083477183 0.984249009846039
3.09901107146927 0.980259325901953
3.1015462243679 0.985867387077271
3.11119400487178 0.980123414771323
3.11554845300908 0.982243619707438
3.11988316682247 0.984285819664027
3.12949999390849 0.968731409076309
3.14290945267774 0.97651645599703
3.14617608555766 0.979720544591433
3.17121235011721 0.990051979853356
3.17432549884301 0.972562425883844
3.22412135560557 0.979242161571539
3.22670676032307 0.985152308723515
3.22823762583094 0.985691567233283
3.22894596736215 0.98777581250371
3.22899816671053 0.978416667755868
3.24084712466588 0.973256998909258
3.24869274451924 0.983681279602121
3.26363109782957 0.982263126959866
3.26494280062718 0.979545409908361
3.27217664416401 0.984468222856631
3.27551413379116 0.978601194182404
3.27577178037818 0.982101011113292
3.2877568510935 0.986360702005776
3.29033090734629 0.970266102050662
3.2954417398048 0.984735689179507
3.31450622284833 0.980216405512867
3.32225913157062 0.992321644148791
3.32795735306142 0.976829449874721
3.32839473401103 0.982646286163098
3.33040474346732 0.976845426546482
3.33265418839896 0.980739381338225
3.33611311101724 0.981216883827153
3.34087237065333 0.984701319512541
3.35172877768159 0.975194684912523
3.35328914139082 0.984530787864874
3.39386116368422 0.976884065345406
3.39742533005062 0.981035547714615
3.40363407071089 0.980836568951355
3.40808488449723 0.982733751890696
3.41076104807395 0.97996760375051
3.41094394245119 0.978126472707939
3.41379024164085 0.958841080876735
3.42384797282245 0.983895664927638
3.42434582094298 0.983334327065424
3.43156517019436 0.981631206486013
3.43236603001016 0.982147310227939
3.43328643641677 0.98027043992965
3.44045231754726 0.973466895380214
3.44226737011648 0.977160635502769
3.44300952055236 0.986036423535835
3.44589523500906 0.985221275420836
3.44906410842006 0.982733374226956
3.45690151265941 0.984518550453783
3.47583248595385 0.966420851303774
3.47615234576982 0.978067226485181
3.48794276718236 0.945914822895769
3.50237823274565 0.98061148162778
3.50359405673934 0.979785031907473
3.53124611556688 0.983740877567993
3.54818974185777 0.978145873990349
3.58257325636424 0.980754055538323
3.60141451592631 0.963111240238686
3.6142109249443 0.983237106403008
3.61793367487007 0.978882289933134
3.62887539099232 0.983015192613775
3.64167752793328 0.976213505001016
3.64909113189349 0.975803785367302
3.66826146816848 0.983177098126874
3.71270603855035 0.970144469891857
3.7228756077762 0.973158805356499
3.7267930173775 0.978394717750816
3.73105877506751 0.971136923815944
3.76536145488467 0.978202549841738
3.78042999910134 0.985043144038619
3.79337096187177 0.979135839877355
3.79537903607238 0.970740808736095
3.85076838354008 0.980656509244141
3.88420179484695 0.964289913161742
3.9149293206751 0.986872672322789
3.91513139142539 0.978960695336606
3.9170808528953 0.983051083096171
3.97055345276468 0.991732576201378
4.0441461021308 0.984315413828502
4.11521533810174 0.978440318401628
4.12134504248109 0.972526499332063
4.3327422865046 0.989030825211135
4.38313514401762 0.979862573689999
4.40296794743456 0.968310939084163
4.81962996095038 0.982963976042486
5.00268682430542 0.963947494359328
};
\addlegendentry{Tensor}
\addplot [semithick, color0, forget plot]
table {%
2.33853895124789 0.896594205279939
2.35530534342027 0.896607281647039
2.40889192192327 0.896649074643704
2.43124458114077 0.896666507826382
2.64439927751083 0.896832750452119
2.8124648649877 0.896963827388418
2.81315941323757 0.89696436907728
2.8178491799041 0.896968026698425
2.85655348991692 0.896998212785025
2.85973443261204 0.897000693651152
2.86054013080652 0.897001322027564
2.88612360370583 0.897021274971519
2.89687947660398 0.897029663642203
2.90742783600007 0.897037890469916
2.91119709283638 0.897040830171288
2.92510490600092 0.897051677088659
2.92736379889279 0.897053438833964
2.93904242566529 0.897062547174586
2.94642166943524 0.897068302360285
2.95069010153344 0.897071631376122
2.95347825235203 0.897073805897823
2.96739269729362 0.897084657987419
2.97754291542565 0.897092574298637
2.98248479730667 0.897096428548315
2.99354777637743 0.897105056735827
3.00373746283297 0.897113003828997
3.06870009706479 0.897163669186474
3.09140083477183 0.897181373840919
3.09901107146927 0.897187309181555
3.1015462243679 0.897189286386288
3.11119400487178 0.897196810838673
3.11554845300908 0.897200206939741
3.11988316682247 0.897203587649706
3.12949999390849 0.897211087961044
3.14290945267774 0.897221546204158
3.14617608555766 0.897224093901378
3.17121235011721 0.897243620069132
3.17432549884301 0.8972460480617
3.22412135560557 0.897284884616183
3.22670676032307 0.897286901013083
3.22823762583094 0.897288094958635
3.22894596736215 0.897288647405088
3.22899816671053 0.897288688116163
3.24084712466588 0.897297929300694
3.24476134146831 0.897300982058573
3.24869274451924 0.897304048220273
3.26363109782957 0.897315698871751
3.26494280062718 0.897316721888936
3.27217664416401 0.897322363674757
3.27551413379116 0.897324966634243
3.27577178037818 0.897325167576779
3.2877568510935 0.897334514917744
3.29033090734629 0.897336522463801
3.2954417398048 0.897340508480634
3.31450622284833 0.897355377164146
3.32225913157062 0.897361423776888
3.32795735306142 0.897365867907459
3.32839473401103 0.897366209027588
3.33040474346732 0.897367776664875
3.33265418839896 0.89736953104157
3.33611311101724 0.897372228708514
3.34087237065333 0.897375940528295
3.35172877768159 0.897384407607094
3.35328914139082 0.897385624558747
3.39386116368422 0.897417267302878
3.39742533005062 0.897420047051039
3.40363407071089 0.897424889343362
3.40808488449723 0.897428360601482
3.41076104807395 0.897430447782611
3.41094394245119 0.897430590424748
3.41379024164085 0.897432810297259
3.42384797282245 0.897440654476482
3.42434582094298 0.897441042755887
3.43156517019436 0.897446673237393
3.43236603001016 0.897447297840279
3.43328643641677 0.89744801567939
3.44045231754726 0.897453604460286
3.44226737011648 0.897455020047698
3.44300952055236 0.897455598862236
3.44589523500906 0.897457849475319
3.44906410842006 0.897460320928425
3.45690151265941 0.89746643344052
3.47583248595385 0.897481197997726
3.47615234576982 0.897481447461316
3.48658939263647 0.897489587474675
3.48794276718236 0.897490642992296
3.50237823274565 0.897501901433888
3.50359405673934 0.897502849673718
3.53124611556688 0.89752441593965
3.54818974185777 0.897537630534364
3.58257325636424 0.897564446766101
3.60141451592631 0.897579141354187
3.6142109249443 0.897589121470372
3.61793367487007 0.89759202490029
3.62887539099232 0.897600558512963
3.64167752793328 0.897610543096443
3.64909113189349 0.897616325080183
3.66826146816848 0.897631276320259
3.71270603855035 0.897665939324198
3.7228756077762 0.897673870727632
3.7267930173775 0.897676925975624
3.73105877506751 0.897680252905649
3.76536145488467 0.897707006093168
3.78042999910134 0.897718758282537
3.79337096187177 0.897728851138416
3.79537903607238 0.897730417266367
3.85076838354008 0.897773616270272
3.88420179484695 0.897799691501912
3.9149293206751 0.897823656371854
3.91513139142539 0.897823813969939
3.9170808528953 0.89782533438492
3.97055345276468 0.897867038487896
4.0441461021308 0.897924434526894
4.11521533810174 0.897979862516979
4.12134504248109 0.897984643167691
4.3327422865046 0.898149515129315
4.38313514401762 0.898188817293865
4.40296794743456 0.898204285202252
4.81962996095038 0.898529246314303
5.00268682430542 0.898672015177206
};
\addplot [semithick, color1, forget plot]
table {%
2.33853895124789 0.982093165701151
2.35530534342027 0.982051037036435
2.40889192192327 0.981916390836119
2.43124458114077 0.981860225641126
2.64439927751083 0.981324634999821
2.8124648649877 0.980902339093088
2.81315941323757 0.980900593912011
2.8178491799041 0.980888810004927
2.85655348991692 0.98079155825972
2.85973443261204 0.980783565552231
2.86054013080652 0.980781541086338
2.88612360370583 0.980717257873769
2.89687947660398 0.980690231751607
2.90742783600007 0.980663727045542
2.91119709283638 0.980654256089844
2.92510490600092 0.980619310134166
2.92736379889279 0.98061363424753
2.94642166943524 0.98056574781913
2.95069010153344 0.980555022593161
2.95347825235203 0.980548016847989
2.96739269729362 0.980513054228743
2.97754291542565 0.980487549926322
2.98248479730667 0.980475132533082
2.99354777637743 0.9804473347498
3.00373746283297 0.980421731275908
3.06870009706479 0.980258500629238
3.09140083477183 0.980201460822593
3.09901107146927 0.980182338693816
3.1015462243679 0.980175968652762
3.11119400487178 0.98015172681791
3.11554845300908 0.980140785460717
3.11988316682247 0.980129893689667
3.12949999390849 0.980105729631009
3.14290945267774 0.980072035883021
3.14617608555766 0.980063827863077
3.17121235011721 0.980000919612779
3.17432549884301 0.979993097250191
3.22412135560557 0.979867975940119
3.22670676032307 0.979861479632065
3.22823762583094 0.979857633049029
3.22894596736215 0.979855853209779
3.22899816671053 0.979855722049251
3.24084712466588 0.979825949348493
3.24869274451924 0.979806235775955
3.26363109782957 0.979768700397351
3.26494280062718 0.979765404501204
3.27217664416401 0.979747228129935
3.27551413379116 0.979738842069293
3.27577178037818 0.979738194684539
3.2877568510935 0.97970807997527
3.29033090734629 0.979701612182335
3.2954417398048 0.979688770269486
3.31450622284833 0.979640867225954
3.32225913157062 0.979621386607298
3.32795735306142 0.979607068770748
3.32839473401103 0.979605969770129
3.33040474346732 0.979600919249207
3.33265418839896 0.97959526710232
3.33611311101724 0.979586575918804
3.34087237065333 0.979574617397767
3.35172877768159 0.97954733866499
3.35328914139082 0.979543417962261
3.39386116368422 0.979441473244133
3.39742533005062 0.979432517616214
3.40363407071089 0.979416917005725
3.40808488449723 0.979405733511996
3.41076104807395 0.979399009155504
3.41094394245119 0.979398549599517
3.41379024164085 0.979391397745797
3.42384797282245 0.979366125833963
3.42434582094298 0.979364874898381
3.43156517019436 0.979346734946688
3.43236603001016 0.979344722638117
3.43328643641677 0.979342409946603
3.44045231754726 0.979324404343463
3.44226737011648 0.979319843687817
3.44300952055236 0.979317978897434
3.44589523500906 0.979310728005556
3.44906410842006 0.979302765624378
3.45690151265941 0.979283072695092
3.47583248595385 0.979235505119523
3.47615234576982 0.979234701412512
3.48794276718236 0.979205075795657
3.50237823274565 0.979168804015629
3.50359405673934 0.979165749032729
3.53124611556688 0.979096268115005
3.54818974185777 0.979053694116751
3.58257325636424 0.978967299170271
3.60141451592631 0.978919957017066
3.6142109249443 0.978887803670089
3.61793367487007 0.978878449571614
3.62887539099232 0.978850956483942
3.64167752793328 0.978818788744498
3.64909113189349 0.978800160691881
3.66826146816848 0.978751991672505
3.71270603855035 0.978640316460282
3.7228756077762 0.978614763534655
3.7267930173775 0.978604920317704
3.73105877506751 0.978594201811681
3.76536145488467 0.978508009977324
3.78042999910134 0.978470147469963
3.79337096187177 0.978437630904917
3.79537903607238 0.978432585246683
3.85076838354008 0.978293409255551
3.88420179484695 0.978209401619276
3.9149293206751 0.978132193021275
3.91513139142539 0.978131685281101
3.9170808528953 0.978126786898205
3.97055345276468 0.97799242709031
4.0441461021308 0.977807511932724
4.11521533810174 0.977628937318517
4.12134504248109 0.977613535301318
4.3327422865046 0.977082360584435
4.38313514401762 0.976955739199439
4.40296794743456 0.97690590560871
4.81962996095038 0.975858965152662
5.00268682430542 0.975399000889574
};
\end{axis}

\end{tikzpicture}

==> figures/mus/admu_rew_th40_mu1.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.462745098039216,0.654901960784314,0.490196078431373}
\definecolor{color1}{rgb}{0.4,0.470588235294118,0.67843137254902}

\begin{axis}[
legend cell align={left},
legend style={at={(0.03,0.03)}, anchor=south west, draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={Lowrank S=20 A=10 R=2 th=40},
x grid style={white!69.01960784313725!black},
xlabel={Incoherence Parameter},
xmajorgrids,
xmin=1.97452271186304, xmax=4.56351653533659,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Average Reward},
ymajorgrids,
ymin=0.517004943176365, ymax=1.01920940004133,
ytick style={color=black}
]
\addplot [only marks, draw=color0, fill=color0, colormap/viridis]
table{%
x                      y
2.10773727918872 0.961592638526264
2.25029522749854 0.967471069285448
2.27219590995873 0.944116814584662
2.31235138291417 0.946594039553198
2.41813137142384 0.899104132547077
2.47186196352973 0.930404644668184
2.48226658659128 0.952271207676458
2.48981511291038 0.845244388859193
2.49988350135547 0.951598264643036
2.50760817282782 0.952344078969386
2.50826388714835 0.908284375076073
2.52380824156355 0.945225389060984
2.53594260531041 0.960812207170544
2.53692885791407 0.961449891340915
2.5386162896392 0.813827127949491
2.54145652335834 0.607886205581111
2.56375916161253 0.9387916721792
2.57581939345437 0.974493411824409
2.58575332342413 0.901899472977276
2.60368627700756 0.838045108831744
2.60368627700757 0.955634407396855
2.60368627700757 0.942637537805773
2.60368627700757 0.952122420424514
2.60368627700758 0.954359913077758
2.60368627700758 0.667083771083648
2.60368627700758 0.948036688522127
2.61282395036398 0.901930281008516
2.62635420869888 0.937705853407171
2.6295983317247 0.897997873577612
2.65790484782034 0.942768756120005
2.66811142083746 0.9256790950657
2.67952464734983 0.98574204188208
2.69937323740091 0.956989083333359
2.70379821584369 0.983107749110406
2.71242715073264 0.866353106965441
2.7246138048709 0.58246623336033
2.73207409607888 0.628507982065746
2.73488492271455 0.966409382961427
2.76475008177618 0.642257966565738
2.78025252044262 0.858873456295494
2.94818178531343 0.979711682999047
3.0074637503095 0.932067268194557
3.02699004291999 0.979207014444986
3.14783640166452 0.848019844256498
3.17418476457404 0.970794966680039
3.18687293051163 0.779541560411298
3.1893349994533 0.920463615857986
3.19719495092785 0.850604274175127
3.20140476998369 0.967525056705756
3.23692883204967 0.89045205560879
3.25062664471254 0.55940433252471
3.26234379430298 0.796760146031483
3.26622792461137 0.931332970713218
3.31010623716258 0.719373404775628
3.31603631780549 0.834940868256853
3.32051683538424 0.982461558475317
3.33231362128898 0.838574622680684
3.34227482640448 0.955984384064372
3.36128168323632 0.965393312331509
3.36866525463896 0.784429816627742
3.38587417365378 0.942601994079041
3.40737389636815 0.962333546711216
3.40937021394963 0.908601336086781
3.41507907427713 0.860787048486992
3.4235333293168 0.626698855014324
3.4379401419049 0.886937534735762
3.45798300631694 0.967712763110733
3.46867235502047 0.972356815264247
3.47051297590839 0.925025777006423
3.47912048320279 0.902038170604955
3.49552024276978 0.939770677229503
3.5079178666439 0.949489465128746
3.51482582586776 0.741105965614382
3.52101607901695 0.934113753283207
3.52482452019852 0.932027658347507
3.53205693359725 0.929561277718458
3.53567570833627 0.972932048733155
3.57019766103987 0.959680752214066
3.5968106081163 0.955535415943164
3.60319363420296 0.9432444098366
3.60604348798807 0.917699682245254
3.60757932398602 0.966827165964829
3.63929892139992 0.908579533924475
3.64053521991206 0.965062010875084
3.65282914521281 0.976223362583378
3.66473898533264 0.965432151990657
3.66617973333047 0.961393289725869
3.70650173167045 0.948285502147399
3.7210173433716 0.979126629183511
3.72386391314108 0.934399763499205
3.72410705062437 0.881645217907425
3.72652841555925 0.940473303533892
3.72699609142572 0.674673456194466
3.72742877397583 0.92639179839568
3.73842529043463 0.966752764632305
3.74729990077924 0.973489235071986
3.74798002219551 0.958584815451437
3.7928538621055 0.894981503812532
3.8123252689493 0.753795546506044
3.81785728812097 0.905749330662503
3.85551492828018 0.986466960386943
3.85972412221641 0.681718955762535
3.87392900536628 0.685681756928028
3.8863089912725 0.968221746344972
3.90568853405406 0.876005722153962
3.91137563011183 0.941939880125672
3.91643713798104 0.960415248990536
3.92902079110774 0.918439704343155
3.94865143382467 0.547949301605292
3.96998027339265 0.978969976030392
3.98013266276186 0.959776904427451
4.00333638937763 0.818337520395251
4.05762777802011 0.971824114492466
4.06076010735151 0.911215163141547
4.08328880468174 0.959454947386707
4.09575847392233 0.899436111035418
4.13245969019548 0.924149678818448
4.26178952539572 0.980306670903351
4.38000905817272 0.950292633633619
4.43030196801091 0.969369925797597
};
\addlegendentry{RMax}
\addplot [only marks, draw=color1, fill=color1, colormap/viridis]
table{%
x                      y
2.10773727918872 0.973535803578934
2.25029522749854 0.978939809342585
2.27219590995873 0.976951817402363
2.31235138291417 0.984888595740123
2.41813137142384 0.983164291299059
2.47186196352973 0.972562425883844
2.48226658659128 0.984284458016046
2.48981511291038 0.982733751890696
2.49988350135547 0.98691353640538
2.50760817282782 0.986482548237323
2.50826388714835 0.97996760375051
2.52380824156355 0.981182619522777
2.53594260531041 0.987102477787357
2.53692885791407 0.984249009846039
2.5386162896392 0.968731409076309
2.54145652335834 0.9852557378269
2.56375916161253 0.985867387077271
2.57581939345437 0.967992191849219
2.58575332342413 0.98027043992965
2.60368627700756 0.981792033406558
2.60368627700757 0.984285819664027
2.60368627700757 0.982243619707438
2.60368627700757 0.981494471564227
2.60368627700758 0.984526761545926
2.60368627700758 0.975837386627959
2.60368627700758 0.974905991589027
2.61282395036398 0.961963577801265
2.62635420869888 0.980225502964051
2.6295983317247 0.983559880263691
2.65790484782034 0.980259325901953
2.66811142083746 0.985691567233283
2.69937323740091 0.984846942352842
2.70379821584369 0.984664588046099
2.71242715073264 0.986180401795894
2.7246138048709 0.973665247245119
2.73207409607888 0.984175713096747
2.73488492271455 0.979545409908361
2.76475008177618 0.990051979853356
2.78025252044262 0.979853479081902
2.94818178531343 0.986036423535835
3.0074637503095 0.981631206486013
3.02699004291999 0.985152308723515
3.14783640166452 0.978601194182404
3.17418476457404 0.979720544591433
3.18687293051163 0.986872672322789
3.1893349994533 0.978416667755868
3.20140476998369 0.984701319512541
3.23692883204967 0.975194684912523
3.25062664471254 0.973158805356499
3.26234379430298 0.980836568951355
3.26622792461137 0.984735689179507
3.31010623716258 0.966420851303774
3.31603631780549 0.979242161571539
3.32051683538424 0.992321644148791
3.33231362128898 0.980123414771323
3.34227482640448 0.97651645599703
3.36128168323632 0.976884065345406
3.36866525463896 0.970266102050662
3.38587417365378 0.983237106403008
3.40737389636815 0.958841080876735
3.40937021394963 0.982263126959866
3.41507907427713 0.981216883827153
3.4235333293168 0.983681279602121
3.4379401419049 0.980739381338225
3.45798300631694 0.982101011113292
3.46867235502047 0.983051083096171
3.47051297590839 0.976829449874721
3.47912048320279 0.982147310227939
3.49552024276978 0.973256998909258
3.5079178666439 0.973466895380214
3.51482582586776 0.986360702005776
3.52101607901695 0.98777581250371
3.52482452019852 0.985221275420836
3.53205693359725 0.945914822895769
3.53567570833627 0.980216405512867
3.57019766103987 0.978145873990349
3.5968106081163 0.983177098126874
3.60319363420296 0.977160635502769
3.60604348798807 0.976845426546482
3.60757932398602 0.984518550453783
3.63929892139992 0.979785031907473
3.64053521991206 0.982733374226956
3.65282914521281 0.983895664927638
3.66473898533264 0.984468222856631
3.66617973333047 0.982646286163098
3.70650173167045 0.983334327065424
3.7210173433716 0.983740877567993
3.72386391314108 0.975803785367302
3.72410705062437 0.984530787864874
3.72652841555925 0.970740808736095
3.72742877397583 0.978202549841738
3.73842529043463 0.980754055538323
3.74729990077924 0.981035547714615
3.74798002219551 0.978126472707939
3.7928538621055 0.98061148162778
3.8123252689493 0.964289913161742
3.81785728812097 0.978067226485181
3.85551492828018 0.984315413828502
3.85972412221641 0.978882289933134
3.87392900536628 0.991732576201378
3.8863089912725 0.970144469891857
3.90568853405406 0.971136923815944
3.91137563011183 0.980656509244141
3.91643713798104 0.963111240238686
3.92902079110774 0.983015192613775
3.94865143382467 0.976213505001016
3.96998027339265 0.978440318401628
3.98013266276186 0.972526499332063
4.00333638937763 0.982963976042486
4.05762777802011 0.978394717750816
4.06076010735151 0.979135839877355
4.08328880468174 0.989030825211135
4.09575847392233 0.978960695336606
4.13245969019548 0.985043144038619
4.26178952539572 0.963947494359328
4.38000905817272 0.968310939084163
4.43030196801091 0.979862573689999
};
\addlegendentry{Tensor}
\addplot [semithick, color0, forget plot]
table {%
2.10773727918872 0.890370366398723
2.25029522749854 0.891236727709791
2.27219590995873 0.891369823788925
2.31235138291417 0.891613858924171
2.41813137142384 0.892256711115975
2.47186196352973 0.89258324574118
2.48226658659128 0.892646477311104
2.48981511291038 0.89269235164667
2.49988350135547 0.892753539832367
2.50760817282782 0.892800484647326
2.50826388714835 0.89280446959187
2.52380824156355 0.892898936630927
2.53594260531041 0.892972680279804
2.53692885791407 0.892978673990494
2.5386162896392 0.892988928947016
2.54145652335834 0.893006189777701
2.56375916161253 0.89314172864556
2.57581939345437 0.893215021775786
2.58575332342413 0.893275392822751
2.60368627700756 0.893384375993189
2.60368627700757 0.893384375993189
2.60368627700757 0.893384375993189
2.60368627700757 0.893384375993189
2.60368627700758 0.893384375993189
2.60368627700758 0.893384375993189
2.60368627700758 0.893384375993189
2.61282395036398 0.893439907983955
2.62635420869888 0.893522134843201
2.6295983317247 0.893541850213065
2.65790484782034 0.89371387619048
2.66811142083746 0.893775904159355
2.67952464734983 0.893845265271815
2.69937323740091 0.893965890257678
2.70379821584369 0.893992781989571
2.71242715073264 0.894045222245847
2.7246138048709 0.894119283676878
2.73207409607888 0.894164621784985
2.73488492271455 0.894181703901262
2.76475008177618 0.894363202152791
2.78025252044262 0.894457414459064
2.94818178531343 0.895477963785181
3.0074637503095 0.895838235530991
3.02699004291999 0.895956901832428
3.14783640166452 0.896691316230509
3.17418476457404 0.896851442007468
3.18687293051163 0.89692855125467
3.1893349994533 0.896943513880756
3.19719495092785 0.896991280827077
3.20140476998369 0.897016864980046
3.23692883204967 0.897232753840336
3.25062664471254 0.897315998970321
3.26234379430298 0.897387207101481
3.26622792461137 0.89741081196018
3.31010623716258 0.897677471748989
3.31603631780549 0.897713510373994
3.32051683538424 0.897740739631498
3.33231362128898 0.897812431733019
3.34227482640448 0.897872968538058
3.36128168323632 0.897988478094694
3.36866525463896 0.898033349956814
3.38587417365378 0.898137932982991
3.40737389636815 0.898268592326642
3.40937021394963 0.898280724461943
3.41507907427713 0.898315418674203
3.4235333293168 0.898366797356116
3.4379401419049 0.898454351260967
3.45798300631694 0.89857615690208
3.46867235502047 0.898641118822948
3.47051297590839 0.898652304749405
3.47912048320279 0.898704614784678
3.49552024276978 0.898804280340813
3.5079178666439 0.898879623889181
3.51482582586776 0.898921605333786
3.52101607901695 0.898959225094015
3.52482452019852 0.898982369970427
3.53205693359725 0.899026323206487
3.53567570833627 0.899048315431154
3.57019766103987 0.899258114215154
3.5968106081163 0.899419847938134
3.60319363420296 0.899458639229077
3.60604348798807 0.899475958523377
3.60757932398602 0.899485292193681
3.63929892139992 0.899678060343952
3.64053521991206 0.899685573647928
3.65282914521281 0.899760286993399
3.66473898533264 0.899832666154457
3.66617973333047 0.899841421950532
3.70650173167045 0.900086469103363
3.7210173433716 0.900174684208402
3.72386391314108 0.900191983544895
3.72410705062437 0.900193461153905
3.72652841555925 0.900208176411275
3.72699609142572 0.90021101859778
3.72742877397583 0.900213648120902
3.73842529043463 0.900280476779208
3.74729990077924 0.900334410068404
3.74798002219551 0.900338543341146
3.7928538621055 0.900611253205717
3.8123252689493 0.900729585952236
3.81785728812097 0.900763205455317
3.85551492828018 0.900992060618335
3.85972412221641 0.901017640972292
3.87392900536628 0.901103967700021
3.8863089912725 0.901179204057922
3.90568853405406 0.901296978522911
3.91137563011183 0.901331540468107
3.91643713798104 0.90136230055301
3.92902079110774 0.901438774648984
3.94865143382467 0.901558075112851
3.96998027339265 0.901687695955679
3.98013266276186 0.901749394636592
4.00333638937763 0.901890409650141
4.05762777802011 0.902220352380109
4.06076010735151 0.902239388350944
4.08328880468174 0.90237630103794
4.09575847392233 0.902452082424526
4.13245969019548 0.902675125153642
4.26178952539572 0.903461095819696
4.38000905817272 0.904179546320877
4.43030196801091 0.904485189266931
};
\addplot [semithick, color1, forget plot]
table {%
2.10773727918872 0.981794818212777
2.25029522749854 0.981513123639655
2.27219590995873 0.981469847880781
2.31235138291417 0.981390500647275
2.41813137142384 0.981181479340071
2.47186196352973 0.981075307664719
2.48226658659128 0.98105474812464
2.48981511291038 0.981039832233072
2.49988350135547 0.981019937092754
2.50760817282782 0.98100467313828
2.50826388714835 0.981003377446473
2.52380824156355 0.980972661794815
2.53594260531041 0.980948684286326
2.53692885791407 0.980946735450716
2.5386162896392 0.980943401084831
2.54145652335834 0.980937788781662
2.56375916161253 0.980893718757949
2.57581939345437 0.980869887734139
2.58575332342413 0.980850258283832
2.60368627700756 0.98081482275909
2.60368627700757 0.98081482275909
2.60368627700757 0.98081482275909
2.60368627700757 0.98081482275909
2.60368627700758 0.98081482275909
2.60368627700758 0.98081482275909
2.60368627700758 0.98081482275909
2.61282395036398 0.980796766712226
2.62635420869888 0.980770030915373
2.6295983317247 0.980763620526743
2.65790484782034 0.980707686837583
2.66811142083746 0.980687518644485
2.69937323740091 0.980625745280206
2.70379821584369 0.980617001520715
2.71242715073264 0.980599950741303
2.7246138048709 0.980575869906976
2.73207409607888 0.980561128368029
2.73488492271455 0.980555574173271
2.76475008177618 0.980496560604874
2.78025252044262 0.980465927778755
2.94818178531343 0.980134099472139
3.0074637503095 0.980016958281336
3.02699004291999 0.979978374317925
3.14783640166452 0.979739581856029
3.17418476457404 0.979687517478488
3.18687293051163 0.979662445656609
3.1893349994533 0.979657580607218
3.20140476998369 0.979633730734956
3.23692883204967 0.979563535171552
3.25062664471254 0.979536468287268
3.26234379430298 0.979513315194149
3.26622792461137 0.979505640150827
3.31010623716258 0.979418936584523
3.31603631780549 0.979407218742375
3.32051683538424 0.979398365237525
3.33231362128898 0.979375054783011
3.34227482640448 0.979355371437003
3.36128168323632 0.979317813878936
3.36866525463896 0.97930322393836
3.38587417365378 0.979269219106268
3.40737389636815 0.97922673564404
3.40937021394963 0.979222790919557
3.41507907427713 0.979211510208857
3.4235333293168 0.979194804596909
3.4379401419049 0.979166336728438
3.45798300631694 0.979126732018903
3.46867235502047 0.979105609860822
3.47051297590839 0.979101972793079
3.47912048320279 0.979084964354604
3.49552024276978 0.979052558421962
3.5079178666439 0.979028060711337
3.51482582586776 0.979014410580651
3.52101607901695 0.979002178637508
3.52482452019852 0.978994653155936
3.53205693359725 0.978980361903648
3.53567570833627 0.978973211203056
3.57019766103987 0.978904995808226
3.5968106081163 0.978852408612246
3.60319363420296 0.978839795749688
3.60604348798807 0.978834164437264
3.60757932398602 0.978831129624607
3.63929892139992 0.978768451685151
3.64053521991206 0.978766008758708
3.65282914521281 0.978741715956513
3.66473898533264 0.978718182106817
3.66617973333047 0.978715335188094
3.70650173167045 0.978635658900349
3.7210173433716 0.978606976044779
3.72386391314108 0.978601351221572
3.72410705062437 0.97860087078179
3.72652841555925 0.978596086163536
3.72742877397583 0.97859430705488
3.73842529043463 0.978572577933169
3.74729990077924 0.978555041698941
3.74798002219551 0.978553697778702
3.7928538621055 0.978465027049867
3.8123252689493 0.978426551540757
3.81785728812097 0.978415620268264
3.85551492828018 0.978341208753542
3.85972412221641 0.978332891384338
3.87392900536628 0.978304822528531
3.8863089912725 0.97828035967054
3.90568853405406 0.97824206568486
3.91137563011183 0.978230827980366
3.91643713798104 0.978220826438429
3.92902079110774 0.978195961133913
3.94865143382467 0.978157170974642
3.96998027339265 0.978115025177593
3.98013266276186 0.978094964051409
4.00333638937763 0.978049113476668
4.05762777802011 0.977941833667095
4.06076010735151 0.977935644182859
4.08328880468174 0.977891127466305
4.09575847392233 0.977866487394002
4.13245969019548 0.97779396577333
4.26178952539572 0.977538409957954
4.38000905817272 0.977304808105409
4.43030196801091 0.97720542929184
};
\end{axis}

\end{tikzpicture}

==> figures/mus/lines/admu_post_th40_kappa_runs=10.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.462745098039216,0.654901960784314,0.490196078431373}
\definecolor{color1}{rgb}{0.4,0.470588235294118,0.67843137254902}

\begin{axis}[
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={Lowrank S=20 A=10 R=4 th=40},
x grid style={white!69.01960784313725!black},
xlabel={Incoherence Parameter},
xmajorgrids,
xmin=4.12098895236893, xmax=16.8552646762906,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Average RewardAfter Exploration},
ymajorgrids,
ymin=0.979010499247573, ymax=1.00215003362737,
ytick style={color=black}
]
\path [draw=color0, fill=color0, opacity=0.25]
(axis cs:4.69981966709264,0.998007865441125)
--(axis cs:4.69981966709264,0.999685406082403)
--(axis cs:6.83849924202389,0.999304279149832)
--(axis cs:8.96266242796467,1.0010982366101)
--(axis cs:10.8539727455871,1.00020238229976)
--(axis cs:12.630767642653,0.999644417750524)
--(axis cs:14.8206329069273,1.00001411684182)
--(axis cs:16.2764339615668,0.998821565882263)
--(axis cs:16.2764339615668,0.996042531870307)
--(axis cs:16.2764339615668,0.996042531870307)
--(axis cs:14.8206329069273,0.996940579697049)
--(axis cs:12.630767642653,0.991705309531345)
--(axis cs:10.8539727455871,0.998171011920978)
--(axis cs:8.96266242796467,0.996364068210376)
--(axis cs:6.83849924202389,0.989470043167455)
--(axis cs:4.69981966709264,0.998007865441125)
--cycle;

\path [draw=color1, fill=color1, opacity=0.25]
(axis cs:4.69981966709264,0.982888288779818)
--(axis cs:4.69981966709264,0.998270324026622)
--(axis cs:6.79566528817633,0.996750775717514)
--(axis cs:8.96266242796467,0.997805139553038)
--(axis cs:10.8258624763279,0.997542281509866)
--(axis cs:12.7624931127918,1.0000501389368)
--(axis cs:14.8438079265618,0.997907140659085)
--(axis cs:16.2764339615668,0.996226239500767)
--(axis cs:16.2764339615668,0.986216394480095)
--(axis cs:16.2764339615668,0.986216394480095)
--(axis cs:14.8438079265618,0.980062296264837)
--(axis cs:12.7624931127918,0.991349295684485)
--(axis cs:10.8258624763279,0.98502642184948)
--(axis cs:8.96266242796467,0.984268968278761)
--(axis cs:6.79566528817633,0.983700343796682)
--(axis cs:4.69981966709264,0.982888288779818)
--cycle;

\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table {%
4.69981966709264 0.998846635761764
6.83849924202389 0.994387161158643
8.96266242796467 0.99873115241024
10.8539727455871 0.99918669711037
12.630767642653 0.995674863640934
14.8206329069273 0.998477348269436
16.2764339615668 0.997432048876285
};
\addlegendentry{RMax}
\addplot [semithick, color1, mark=square*, mark size=3, mark options={solid}]
table {%
4.69981966709264 0.99057930640322
6.79566528817633 0.990225559757098
8.96266242796467 0.991037053915899
10.8258624763279 0.991284351679673
12.7624931127918 0.995699717310642
14.8438079265618 0.988984718461961
16.2764339615668 0.991221316990431
};
\addlegendentry{GWSM}
\end{axis}

\end{tikzpicture}

==> figures/mus/lines/admu_rew_line_th40_mu1.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.462745098039216,0.654901960784314,0.490196078431373}
\definecolor{color1}{rgb}{0.4,0.470588235294118,0.67843137254902}

\begin{axis}[
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={Lowrank S=20 A=10 R=2 th=40},
x grid style={white!69.01960784313725!black},
xlabel={Incoherence Parameter},
xmajorgrids,
xmin=2.47431188301166, xmax=4.44703613469382,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Average Reward},
ymajorgrids,
ymin=0.769835492388085, ymax=1.01392744713536,
ytick style={color=black}
]
\path [draw=color0, fill=color0, opacity=0.25]
(axis cs:2.5668697541833,0.783796361927287)
--(axis cs:2.5668697541833,1.00110962513943)
--(axis cs:3.29992794386917,0.985644081607868)
--(axis cs:3.7731935513142,1.00283235828321)
--(axis cs:4.35736685052645,0.979058909425267)
--(axis cs:4.35736685052645,0.954253910797778)
--(axis cs:4.35736685052645,0.954253910797778)
--(axis cs:3.7731935513142,0.810526794042699)
--(axis cs:3.29992794386917,0.780930581240234)
--(axis cs:2.5668697541833,0.783796361927287)
--cycle;

\path [draw=color1, fill=color1, opacity=0.25]
(axis cs:2.56398116717904,0.974926482195629)
--(axis cs:2.56398116717904,0.986655344169094)
--(axis cs:3.30335237696722,0.985877290248571)
--(axis cs:3.77422016153395,0.986634874045265)
--(axis cs:4.35736685052645,0.977421577420518)
--(axis cs:4.35736685052645,0.963992427335142)
--(axis cs:4.35736685052645,0.963992427335142)
--(axis cs:3.77422016153395,0.97137730590404)
--(axis cs:3.30335237696722,0.973069209279916)
--(axis cs:2.56398116717904,0.974926482195629)
--cycle;

\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table {%
2.5668697541833 0.892452993533359
3.29992794386917 0.883287331424051
3.7731935513142 0.906679576162956
4.35736685052645 0.966656410111522
};
\addlegendentry{RMax}
\addplot [semithick, color1, mark=square*, mark size=3, mark options={solid}]
table {%
2.56398116717904 0.980790913182362
3.30335237696722 0.979473249764243
3.77422016153395 0.979006089974653
4.35736685052645 0.97070700237783
};
\addlegendentry{GWSM}
\end{axis}

\end{tikzpicture}

==> figures/mus/lines/admu_rew_th40_kappa_runs=10.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}[scale=0.3]

\definecolor{color0}{rgb}{0.462745098039216,0.654901960784314,0.490196078431373}
\definecolor{color1}{rgb}{0.4,0.470588235294118,0.67843137254902}

\begin{axis}[
legend cell align={left},
legend style={at={(0.03,0.03)}, anchor=south west, draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={\textbf{(c) \avgrew versus $\kappa$}},
x grid style={white!69.01960784313725!black},
xlabel={$\kappa$},
xmajorgrids,
xmin=4.12098895236893, xmax=16.8552646762906,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Average Reward},
ymajorgrids,
ymin=0.554034059609227, ymax=1.05350660506006,
ytick style={color=black}
]
\path [draw=color0, fill=color0, opacity=0.25]
(axis cs:4.69981966709264,0.821818561182312)
--(axis cs:4.69981966709264,1.00995363808451)
--(axis cs:6.79566528817633,0.914140082006651)
--(axis cs:8.96266242796467,1.00349524185089)
--(axis cs:10.8258624763279,1.03080330753957)
--(axis cs:12.7624931127918,0.947422398450315)
--(axis cs:14.8206329069273,0.968517860817394)
--(axis cs:16.2764339615668,0.966275837063459)
--(axis cs:16.2764339615668,0.737779143909527)
--(axis cs:16.2764339615668,0.737779143909527)
--(axis cs:14.8206329069273,0.93058366073669)
--(axis cs:12.7624931127918,0.64953386692571)
--(axis cs:10.8258624763279,0.719353877861491)
--(axis cs:8.96266242796467,0.855391767707752)
--(axis cs:6.79566528817633,0.57673735712972)
--(axis cs:4.69981966709264,0.821818561182312)
--cycle;

\path [draw=color1, fill=color1, opacity=0.25]
(axis cs:4.69981966709264,0.971977255220816)
--(axis cs:4.69981966709264,0.986655700140626)
--(axis cs:6.79566528817633,0.984142784918904)
--(axis cs:8.96266242796467,0.985086889951492)
--(axis cs:10.8258624763279,0.984453115649103)
--(axis cs:12.7624931127918,0.999412931102172)
--(axis cs:14.8206329069273,1.02660307411299)
--(axis cs:16.2764339615668,0.978995736884425)
--(axis cs:16.2764339615668,0.964197833823263)
--(axis cs:16.2764339615668,0.964197833823263)
--(axis cs:14.8206329069273,0.86487969774073)
--(axis cs:12.7624931127918,0.943329303821003)
--(axis cs:10.8258624763279,0.973110488250473)
--(axis cs:8.96266242796467,0.972943612999604)
--(axis cs:6.79566528817633,0.96838232107418)
--(axis cs:4.69981966709264,0.971977255220816)
--cycle;

\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table {%
4.69981966709264 0.915886099633409
6.79566528817633 0.745438719568185
8.96266242796467 0.929443504779319
10.8258624763279 0.87507859270053
12.7624931127918 0.798478132688012
14.8206329069273 0.949550760777042
16.2764339615668 0.852027490486493
nan nan
};
\addlegendentry{RMax}
\addplot [semithick, color1, mark=square*, mark size=3, mark options={solid}]
table {%
4.69981966709264 0.979316477680721
6.79566528817633 0.976262552996542
8.96266242796467 0.979015251475548
10.8258624763279 0.978781801949788
12.7624931127918 0.971371117461587
14.8206329069273 0.945741385926859
16.2764339615668 0.971596785353844
nan nan
};
\addlegendentry{\ourmod}
\end{axis}

\end{tikzpicture}

==> figures/rank/ranks.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}[scale=0.45]

\definecolor{color0}{rgb}{0.462745098039216,0.654901960784314,0.490196078431373}
\definecolor{color1}{rgb}{0.4,0.470588235294118,0.67843137254902}

\begin{axis}[
legend cell align={left},
legend style={at={(0.03,0.97)}, anchor=north west, draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={Lowrank S=20 A=10 runs3},
x grid style={white!69.01960784313725!black},
xlabel={Rank},
xmajorgrids,
xmin=1.6, xmax=10.4,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Average Rewards After Exploration},
ymajorgrids,
ymin=0.979245885280084, ymax=1,
ytick style={color=black},
yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=3,
            /pgf/number format/fixed zerofill
        },
        scaled y ticks=false
]
\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table {%
2 0.994541769347971
4 0.992261485057248
6 0.996544639672535
8 0.999340255437126
10 0.998571011805271
};
\addlegendentry{RMax}
\addplot [semithick, color1, mark=square*, mark size=3, mark options={solid}]
table {%
2 0.99134061140967
4 0.985585342310768
6 0.987502665125885
8 0.980202760049467
10 0.980921695968578
};
\addlegendentry{\ourmod}
\end{axis}

\end{tikzpicture}

==> figures/rank/ranks_avg_shade_runs=3.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}[scale=0.35]

\definecolor{color0}{rgb}{0.462745098039216,0.654901960784314,0.490196078431373}
\definecolor{color1}{rgb}{0.4,0.470588235294118,0.67843137254902}

\begin{axis}[
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={Lowrank S=20 A=10},
x grid style={white!69.01960784313725!black},
xlabel={Rank},
xmajorgrids,
xmin=1.6, xmax=10.4,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Average Reward},
ymajorgrids,
ymin=0.831505390445296, ymax=1.00227604476485,
ytick style={color=black},
ytick={0.82,0.84,0.86,0.88,0.9,0.92,0.94,0.96,0.98,1,1.02},
yticklabels={0.82,0.84,0.86,0.88,0.90,0.92,0.94,0.96,0.98,1.00,1.02}
]
\path [draw=color0, fill=color0, opacity=0.25]
(axis cs:2,0.839267692914367)
--(axis cs:2,0.906166888114161)
--(axis cs:4,0.915976883459504)
--(axis cs:6,0.940918667768202)
--(axis cs:8,0.918345212110289)
--(axis cs:10,0.938528590197248)
--(axis cs:10,0.868995871088772)
--(axis cs:10,0.868995871088772)
--(axis cs:8,0.842888949454121)
--(axis cs:6,0.874304734075864)
--(axis cs:4,0.844158280251279)
--(axis cs:2,0.839267692914367)
--cycle;

\path [draw=color1, fill=color1, opacity=0.25]
(axis cs:2,0.9616416023461)
--(axis cs:2,0.994513742295777)
--(axis cs:4,0.987838222110755)
--(axis cs:6,0.987903349364471)
--(axis cs:8,0.981281435352508)
--(axis cs:10,0.981158989463309)
--(axis cs:10,0.947853734356243)
--(axis cs:10,0.947853734356243)
--(axis cs:8,0.946773182679961)
--(axis cs:6,0.954020589530608)
--(axis cs:4,0.949875206451416)
--(axis cs:2,0.9616416023461)
--cycle;

\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table {%
2 0.872619992794782
4 0.880739354393136
6 0.908045460328385
8 0.882345177089358
10 0.90387238947617
};
\addlegendentry{RMax}
\addplot [semithick, color1, mark=square*, mark size=3, mark options={solid}]
table {%
2 0.978174498822591
4 0.969136377978411
6 0.971590276307643
8 0.964686823215829
10 0.965165920849133
};
\addlegendentry{\ourmod}
\end{axis}

\end{tikzpicture}

==> figures/rank/ranks_post_shade_runs=3.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}[scale=0.35]

\definecolor{color0}{rgb}{0.462745098039216,0.654901960784314,0.490196078431373}
\definecolor{color1}{rgb}{0.4,0.470588235294118,0.67843137254902}

\begin{axis}[
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={Lowrank S=20 A=10},
x grid style={white!69.01960784313725!black},
xlabel={Rank},
xmajorgrids,
xmin=1.6, xmax=10.4,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Average RewardAfter Exploration},
ymajorgrids,
ymin=0.969564836529003, ymax=1.01047004072818,
ytick style={color=black}
]
\path [draw=color0, fill=color0, opacity=0.25]
(axis cs:2,0.982953841674973)
--(axis cs:2,1.00631692347973)
--(axis cs:4,1.00551531450849)
--(axis cs:6,1.0060185810387)
--(axis cs:8,1.00861071326458)
--(axis cs:10,1.00646155087227)
--(axis cs:10,0.990537808622193)
--(axis cs:10,0.990537808622193)
--(axis cs:8,0.989878625511628)
--(axis cs:6,0.986362946579117)
--(axis cs:4,0.979164255257108)
--(axis cs:2,0.982953841674973)
--cycle;

\path [draw=color1, fill=color1, opacity=0.25]
(axis cs:2,0.979870233553493)
--(axis cs:2,1.00358175382883)
--(axis cs:4,0.998610893092724)
--(axis cs:6,0.997094475334133)
--(axis cs:8,0.989687627622677)
--(axis cs:10,0.989733773321687)
--(axis cs:10,0.972194179692928)
--(axis cs:10,0.972194179692928)
--(axis cs:8,0.971424163992602)
--(axis cs:6,0.977967474486856)
--(axis cs:4,0.972639022751748)
--(axis cs:2,0.979870233553493)
--cycle;

\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table {%
2 0.99477707109573
4 0.992377239606509
6 0.996404838710103
8 0.999312866902246
10 0.998649710341815
};
\addlegendentry{RMax}
\addplot [semithick, color1, mark=square*, mark size=3, mark options={solid}]
table {%
2 0.991667394345888
4 0.985545813078726
6 0.987360535208919
8 0.980559232782521
10 0.980992236368446
};
\addlegendentry{\ourmod}
\end{axis}

\end{tikzpicture}

==> figures/rank/ranks_times_shade_runs=3.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}[scale=0.35]

\definecolor{color0}{rgb}{0.462745098039216,0.654901960784314,0.490196078431373}
\definecolor{color1}{rgb}{0.4,0.470588235294118,0.67843137254902}

\begin{axis}[
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={Lowrank S=20 A=10 runs 3},
x grid style={white!69.01960784313725!black},
xlabel={Rank},
xmajorgrids,
xmin=1.6, xmax=10.4,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Non-optimal Episodes},
ymajorgrids,
ymin=1836.66570244121, ymax=374551.084084765,
ytick style={color=black}
]
\path [draw=color0, fill=color0, opacity=0.25]
(axis cs:2,84683.1470538259)
--(axis cs:2,357609.519612841)
--(axis cs:4,268096.072651682)
--(axis cs:6,212351.630539672)
--(axis cs:8,244971.070453363)
--(axis cs:10,171606.585192004)
--(axis cs:10,89293.4148079962)
--(axis cs:10,89293.4148079962)
--(axis cs:8,79791.596213304)
--(axis cs:6,38083.7027936612)
--(axis cs:4,89580.594014985)
--(axis cs:2,84683.1470538259)
--cycle;

\path [draw=color1, fill=color1, opacity=0.25]
(axis cs:2,18915.7072412173)
--(axis cs:2,28146.9594254494)
--(axis cs:4,29780.4118961851)
--(axis cs:6,28257.769825635)
--(axis cs:8,23482.8055356586)
--(axis cs:10,24977.5957384762)
--(axis cs:10,19975.7375948571)
--(axis cs:10,19975.7375948571)
--(axis cs:8,20651.8611310081)
--(axis cs:6,18778.230174365)
--(axis cs:4,22768.2547704815)
--(axis cs:2,18915.7072412173)
--cycle;

\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table {%
2 221146.333333333
4 178838.333333333
6 125217.666666667
8 162381.333333333
10 130450
};
\addlegendentry{RMax}
\addplot [semithick, color1, mark=square*, mark size=3, mark options={solid}]
table {%
2 23531.3333333333
4 26274.3333333333
6 23518
8 22067.3333333333
10 22476.6666666667
};
\addlegendentry{\ourmod}
\end{axis}

\end{tikzpicture}

==> include/poster/supp_macros.tex <==
\newcommand*{\mytensor}[1]{\bm{\mathcal{#1}}}
\newcommand*{\mymatrix}[1]{\bm{#1}}
\newcommand*{\myvector}[1]{\bm{#1}}
\newcommand*{\noise}[1]{\widehat{#1}}
\newcommand*{\mm}{\mymatrix}
\newcommand*{\mv}{\myvector}
\newcommand{\mt}{\mytensor}
\newcommand*{\mmCols}[2]{\mm{#1}_{[#2]}}

% names
\newcommand{\ourmod}{{GIM}\xspace}
\newcommand{\ourmodfull}{{Greedy Inference Model}\xspace}
\newcommand{\dmname}{{dynamic matrix}\xspace}
\newcommand{\dmnames}{{dynamic matrices}\xspace}
\newcommand{\avgrew}{{AvgReward}\xspace}
\newcommand{\pavgrew}{{PostAvgReward}\xspace}
\newcommand{\numepi}{{TotalEps}\xspace}
\newcommand{\walkname}{{$\beta$-curious walking}\xspace}

% about dynamic matrices
\newcommand{\states}{\mathcal{S}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\dmat}{\mymatrix{M}}
\newcommand{\dmats}{M}
\newcommand{\admat}{\mymatrix{\hat{M}}}
\newcommand{\rdmat}{\mymatrix{\widetilde{M}}}
\newcommand{\rdmats}{\widetilde{M}}
\newcommand{\dmatset}{\{\mymatrix{M}^k\}_{k=1}^{S+1}}
\newcommand{\admatset}{\{\mymatrix{\hat{M}}^k\}_{k=1}^{S+1}}
\newcommand{\rdmatset}{\{\mymatrix{\widetilde{M}}^k\}_{k=1}^{S+1}}
\newcommand{\krange}{1,2,\cdots,S+1}


% about mask
\newcommand{\mask}{\mymatrix{P}^\mathcal{K}}
\newcommand{\masks}{P^\mathcal{K}}
\newcommand{\kset}{\mathcal{K}}
\newcommand{\nkset}{\bar{\mathcal{K}}}

% about noise
\newcommand{\noiset}{\mytensor{Z}}
\newcommand{\noisem}{\mymatrix{Z}}
\newcommand{\noises}{Z}

\newcommand{\fraction}{\rho}

\newcommand{\minsa}{M_{in}}
\newcommand{\maxsa}{M_{ax}}

\DeclareMathOperator*{\minimize}{\text{minimize}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% author comments

\iffalse
\newcommand{\fhcomment}{\textcolor[rgb]{1,0,0}{F: }\textcolor[rgb]{1,0,0}}


\newcommand{\grcomment}{}
\newcommand{\jccomment}{}
\newcommand{\fhcomment}{}
\newcommand{\yycomment}{}


% math commands
\newcommand{\F}{\mathcal{F}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\text{Var}}

\newcommand{\ff}{{\frac{\sqrt{\epsilon}}{2}}}
\newcommand\inner[1]{\langle #1 \rangle}
\newcommand\supp{\operatorname{supp}}

\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}

\newcommand{\name}{{strict saddle}}
\newcommand{\bigname}{{Strict saddle}}


\newcommand{\Hess}{\nabla^2}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\tlO}{\tilde{O}}
\newcommand{\tlOmega}{\tilde{\Omega}}
\newcommand{\nameCQ}{ $\alpha_c$-RLICQ }
\newcommand{\BigC}{\mathfrak{S}}

\setmainfont{Corbel}  % This was the font used in the powerpoint template


\setlength{\parskip}{0.3em}

\def\Pbb{{\mathbb P}}
\DeclareMathOperator{\Cum}{C_3}
\def\Ebb{{\mathbb E}}
\DeclareMathOperator{\flatten}{unfold}
\def\tha{{\mbox{\tiny th}}}
\newcommand{\CToep}{{\mathcal{F}}}





\DeclareMathOperator*{\argmax}{argmax}




\fi

\newcommand{\ft}{\frametitle}
\newcommand{\bef}{\begin{frame}}
\newcommand{\eef}{\end{frame}} %strange doesnt work
\newcommand{\beb}{\begin{block}}
\newcommand{\eeb}{\end{block}}
\newcommand{\becs}{\begin{columns}}
\newcommand{\eecs}{\end{columns}}
\newcommand{\bec}{\begin{column}}
\newcommand{\eec}{\end{column}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}

%presentation specs
\def\tcr{\textcolor{red}}
\def\tcb{\textcolor{blue}}
\def\tcg{\textcolor{green}}
\def\tcw{\textcolor{white}}
\def\tcm{\textcolor{magenta}}
\def\tccyan{\textcolor{cyan}}
\def\tcv{\textcolor{violet}}
\definecolor{dkr}{rgb}{0.6,0.2,0.2}
\definecolor{dkg}{rgb}{0,0.5,0}
\definecolor{dkb}{rgb}{0.0,0.1,0.7}

\def\tcdkb{\textcolor{dkb}}
\def\tcdkg{\textcolor{dkg}}
\def\tcdkr{\textcolor{dkr}}
\def\tcblack{\textcolor{black}}


==> include/poster/supp_packages.tex <==
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{algorithmicx,algpseudocode}
\usepackage{multirow}
%\usepackage{tikz}
%\usetikzlibrary{bayesnet}
%\usepackage{fontspec}
 \usepackage{color}
 \usepackage{psfrag}
 \usepackage{natbib}
 \usepackage{epstopdf}
 \usepackage{subfig}
 \usepackage{hyperref}
\usepackage{siunitx}
\usepackage[labelformat=empty]{caption}  % Disable figure numbering and labels

\usepackage{tikz}
\usetikzlibrary{fit}
\usetikzlibrary{calc,shapes}
\usetikzlibrary{decorations.pathmorphing} % noisy shapes
\usetikzlibrary{fit}					% fitting shapes to coordinates
\usetikzlibrary{backgrounds}	% drawing the background after the foreground
%pgfplots
\usepackage[utf8]{inputenc}
% \usepackage{fontspec}  % optional
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{dateplot}

\usepackage{tcolorbox}
\usepackage{pgfpages}

==> include/talks/supp_macros.tex <==
\definecolor{mygray}{gray}{0.6}
\newcommand{\mycite}[1]{\textcolor{mygray}{\scriptsize{#1}}}

%\newcommand{\myvector}[1]{\ensuremath{\bm{#1}}}
%\newcommand{\mymatrix}[1]{\ensuremath{\bm{#1}}}
%\newcommand{\mytensor}[1]{\bm{\mathcal{#1}}}
%\newcommand{\tensor}[1]{\bm{\mathcal{#1}}}
\newcommand\Dir{\operatorname{Dir}}
\def\tl{\tilde}

\renewcommand\t{{\scriptscriptstyle\top}}

\newcommand\iideq{\stackrel{\mathclap{\normalfont\mbox{\scriptsize{iid}}}}{=}}
\newcommand\iidsim{\stackrel{\mathclap{\normalfont\mbox{\scriptsize{iid}}}}{\sim}}
\newcommand\aseq{\stackrel{\mathclap{\normalfont\mbox{\scriptsize{a.s.}}}}{=}}
\newcommand\whpeq{\stackrel{\mathclap{\normalfont\mbox{\scriptsize{w.h.p.}}}}{\ =\ }}



%\newcommand{\vectorSub}[2]{\ensuremath{\bm{#1}}_{#2}}	
%\newcommand{\vectorSup}[2]{\ensuremath{\bm{#1}}^{(#2)}}
%\newcommand{\vectorInd}[3]{\ensuremath{\bm{#1}}_{#2}^{(#3)}}
%\newcommand{\matrixSub}[2]{\ensuremath{\bm{#1}}_{#2}}	
%\newcommand{\matrixSup}[2]{\ensuremath{\bm{#1}}^{(#2)}}
%\newcommand{\matrixInd}[3]{\ensuremath{\bm{#1}}_{#2}^{(#3)}}
%\newcommand{\tensorSub}[2]{\ensuremath{\bm{\mathcal{#1}}}_{#2}}	
%\newcommand{\tensorSup}[2]{\ensuremath{\bm{\mathcal{#1}}}^{(#2)}}
%\newcommand{\tensorInd}[3]{\ensuremath{\bm{\mathcal{#1}}}_{#2}^{(#3)}}

%\newcommand{\swapaxes}{\mathsf{swapaxes}}
%\newcommand{\flipaxis}{\mathsf{flipaxis}}

%\newcommand\cpeq{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny cp}}}{=}}}
%\newcommand\tkeq{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny tk}}}{=}}}
%\newcommand\tteq{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny tt}}}{=}}}


\newcommand\asymptoticeq{\stackrel{\mathclap{\normalfont\mbox{\scriptsize{\ensuremath{n\!\!\rightarrow\!\!\infty}}}}}{\quad =\quad }}

\newcommand{\mle}{\ensuremath{{\mathsf{mle}}}}
\DeclareMathOperator{\Triples}{T}
\newcommand\inner[1]{\ensuremath{\langle #1 \rangle}}
 \def\hC{\widehat{C}}
\def\hE{\widehat{E}}
% \def\hF{\widehat{F}}
 \def\hG{\widehat{G}}
  \def\hG{\widehat{J}}
 \def\hk{\widehat{k}}
\def\hl{\widehat{l}}
 \def\hSigma{{\widehat{\Sigma}}}
\DeclareMathOperator{\poly}{poly}

 \def\0{{\bf 0}}

\def\leqst{{\overset{st}{\leq}}}
\def\geqst{{\overset{st}{\geq}}}
\def\geqrh{{\overset{rh}{\geq}}}
\def\geqlr{{\overset{lr}{\geq}}}
\def\eqlr{{\overset{lr}{=}}}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclareMathOperator{\atanh}{atanh}
\def\tilomega{{\widetilde{\omega}}}
\def\edoc{\end{document}}

\DeclareMathOperator{\rank}{Rank}
  \DeclareMathOperator{\tw}{tw}
\def\Tsawi{{T_{\mathrm{saw}}(i;G)}}
\DeclareMathOperator{\Deg}{Deg}
\DeclareMathOperator{\aug}{Aug}
\DeclareMathOperator{\watts}{Watts}
\DeclareMathOperator{\girth}{Girth}
\DeclareMathOperator{\PL}{PL}
\DeclareMathOperator{\LP}{LP}
\DeclareMathOperator{\ER}{ER}
\DeclareMathOperator{\reg}{Reg}
%mbox - function definitions
\def\tha{\mbox{\tiny th}}
\DeclareMathOperator{\Det}{Det}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\Cov}{\mbox{Cov}}
\newcommand{\Poiss}{\mbox{${\mbox{Poiss}}$}}
\newcommand{\Diag}{\mbox{${\mbox{Diag}}$}}
\newcommand{\Diam}{\mbox{${\mbox{Diam}}$}}
\def\erf{\mbox{erf}}
\def\erfc{\mbox{erfc}}
\def\qfunc{\mbox{Q}}
\def\myexp{\mbox{e}}
\def\snr{\mbox{\tiny SNR}}
\def\signum{\mbox{sgn}}
\def\Card{\mbox{\small N}}
\def\plim{\mbox{p\,}\lim}
\def\convd{\overset{d}\rightarrow}
\def\convp{\overset{p}\rightarrow}
\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%text abbreviations
\def\etal{{et al. \/}}
\def\viz{{viz.,\ \/}}
\def\ie{{i.e.,\ \/}}
\def\eg{{e.g.,  }}
\def\etc{{etc.,  }}
\def\ifff{{iff  }}
\def\as{{a.s.  }}
\def\st{{s.t.  }}
\def\wpone{{w.p.}\,1\,\,}
\def\nn{\nonumber}
\def\qed{\hfill$\Box$}
\def\complx{\mathbb{C}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LDP
%
%\def\EGnp{\tilde{E}^{\mbox{\tiny NPD}}(\lambda)}
%\def\EGB{\tilde{E}^{\mbox{\tiny BD}}(\lambda)}
%\def\EGFI{\tilde{E}^{\mbox{\tiny MLE}}(\lambda,\theta)}
%\def\trueEGnp{{E}^{\mbox{\tiny NPD}}(\lambda)}
%\def\trueEGB{{E}^{\mbox{\tiny BD}}(\lambda)}
%\def\trueEFI{{E}^{\mbox{\tiny MLE}}(\lambda,\theta)}
%\def\thetaml{\hat{\theta}_{{\mbox{\tiny MLE}}}}
%\def\nustar{\nu_{*}}
%\def\trueEB{{E}^{\mbox{\tiny D}}(\lambdabf)}
%\def\trueEF{{E}^{\mbox{\tiny E}}(\lambdabf)}
%\def\tilDlambdagamma{\tilde{D}_{\lambda,\gamma}}
%\def\tilClambdagamma{\tilde{C}_{\lambda,\gamma}}
%\def\tilD{\tilde{D}}
%\def\tilC{\tilde{C}}
%\def\delpj{\Delta p_\theta(j)}
%\def\mindet{\hat{\theta}_{\mbox{\tiny mrd}}}
%\def\minsumrate{\hat{\theta}_{\mbox{\tiny msd}}}
%\def\sprt{\mathbb{E}_{\theta_i}N_{\mbox{\tiny sprt}}(\lambda)}
%\def\smst{\mathbb{E}_{\theta_i}N_{\mbox{\tiny smst}}(\lambda)}
%\def\sprtzero{\mathbb{E}_{\theta_0}N_{\mbox{\tiny sprt}}(\lambda)}
%\def\smstzero{\mathbb{E}_{\theta_0}N_{\mbox{\tiny smst}}(\lambda)}
%\def\sprtone{\mathbb{E}_{\theta_1}N_{\mbox{\tiny sprt}}(\lambda)}
%\def\smstone{\mathbb{E}_{\theta_1}N_{\mbox{\tiny smst}}(\lambda)}
%\def\nsprt{N_{\mbox{\tiny sprt}}}
%\def\nsmst{N_{\mbox{\tiny smst}}}
%\def\diffseq{\mathbb{E}_{\theta_i}(N_{\mbox{\tiny sprt}}-N_{\mbox{\tiny
%smst}})(\lambda)}
%\def\xij{\{X_{i,j}\}}
%\def\xioneseq{\{X_{i,1}\}_{i=1}^\infty}
%\def\xinseq{\{X_{i,n}\}_{i=1}^\infty}
%\def\xij{X_{i,j}}
%\def\hione{H_{i,1}}
%\def\hitwo{H_{i,2}}
%\def\hij{H_{i,j}}
%\def\snrt{\mbox{\scriptsize{SNR}}_t}
%\def\snrr{\mbox{\small{SNR}}_r}
%\def\plim{\mbox{p}\lim}
%\def\convd{\overset{d}\rightarrow}
%\def\convp{\overset{p}\rightarrow}
%\def\convweak{\Rightarrow}
%%\def\bfptheta{\mathbf{p}_{\theta}}
%\def\pt{\mathbf{p}_{\theta}}
%\def\pti{\mathbf{p}_{\theta_i}}
%\def\ptzero{\mathbf{p}_{\theta_0}}
%\def\ptone{\mathbf{p}_{\theta_1}}
%\def\pthetai{p_{\theta_i}}
%\def\ptheta{p_{\theta}}
%\def\conv{{ \rightarrow}}
%\def\balle{\mathcal{B}_\epsilon}
%\def\thetai{\theta_i}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%presentation specs
\def\tcr{\textcolor{red}}
\def\tcb{\textcolor{blue}}
\def\tcg{\textcolor{green}}
\def\tcw{\textcolor{white}}
\def\tcm{\textcolor{magenta}}
\def\tccyan{\textcolor{cyan}}
\def\tcv{\textcolor{violet}}
\definecolor{dkr}{rgb}{0.6,0.2,0.2}
\definecolor{dkg}{rgb}{0,0.5,0}
\definecolor{dkb}{rgb}{0.0,0.1,0.7}

\def\tcdkb{\textcolor{dkb}}
\def\tcdkg{\textcolor{dkg}}
\def\tcdkr{\textcolor{dkr}}
\def\tcblack{\textcolor{black}}

%beamer
\newcommand{\ft}{\frametitle}
\newcommand{\bef}{\begin{frame}}
\newcommand{\eef}{\end{frame}}%strange doesnt work
\newcommand{\beb}{\begin{block}}
\newcommand{\eeb}{\end{block}}
\newcommand{\becs}{\begin{columns}}
\newcommand{\eecs}{\end{columns}}
\newcommand{\bec}{\begin{column}}
\newcommand{\eec}{\end{column}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\mathscr

\newcommand{\Amsc}{\mathscr{A}}
\newcommand{\Cmsc}{\mathscr{C}}
\newcommand{\Dmsc}{\mathscr{D}}
\newcommand{\Emsc}{\mathscr{E}}
\newcommand{\Fmsc}{\mathscr{F}}
\newcommand{\Gmsc}{\mathscr{G}}
\newcommand{\Hmsc}{\mathscr{H}}
\newcommand{\Kmsc}{\mathscr{K}}
\newcommand{\Nmsc}{\mathscr{N}}
\newcommand{\Pmsc}{\mathscr{P}}
\newcommand{\Qmsc}{\mathscr{Q}}
\newcommand{\Rmsc}{\mathscr{R}}
\newcommand{\Smsc}{\mathscr{S}}
\newcommand{\Tmsc}{\mathscr{T}}
\newcommand{\Umsc}{\mathscr{U}}
\newcommand{\Xmsc}{\mathscr{X}}
\newcommand{\Ymsc}{\mathscr{Y}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%bold alphabets
\def\bfzero{{\mathbf{0}}}
\def\bfone{{\mathbf{1}}}
\def\bfa{{\mathbf a}}
\def\bfb{{\mathbf b}}
\def\bfc{{\mathbf c}}
\def\bfd{{\mathbf d}}
\def\bfe{{\mathbf e}}
\def\bff{{\mathbf f}}
\def\bfg{{\mathbf g}}
\def\bfh{{\mathbf h}}
\def\bfi{{\mathbf i}}
\def\bfj{{\mathbf j}}
\def\bfk{{\mathbf k}}
\def\bfl{{\mathbf l}}
\def\bfm{{\mathbf m}}
\def\bfn{{\mathbf n}}
\def\bfo{{\mathbf o}}
\def\bfp{{\mathbf p}}
\def\bfq{{\mathbf q}}
\def\bfr{{\mathbf r}}
\def\bfs{{\mathbf s}}
\def\bft{{\mathbf t}}
\def\bfu{{\mathbf u}}
\def\bfv{{\mathbf v}}
\def\bfw{{\mathbf w}}
\def\bfx{{\mathbf x}}
\def\bfy{{\mathbf y}}
\def\bfz{{\mathbf z}}
%bold caps
\def\bfA{{\mathbf A}}
\def\bfB{{\mathbf B}}
\def\bfC{{\mathbf C}}
\def\bfD{{\mathbf D}}
\def\bfE{{\mathbf E}}
\def\bfF{{\mathbf F}}
\def\bfG{{\mathbf G}}
\def\bfH{{\mathbf H}}
\def\bfI{{\mathbf I}}
\def\bfJ{{\mathbf J}}
\def\bfK{{\mathbf K}}
\def\bfL{{\mathbf L}}
\def\bfM{{\mathbf M}}
\def\bfN{{\mathbf N}}
\def\bfO{{\mathbf O}}
\def\bfP{{\mathbf P}}
\def\bfQ{{\mathbf Q}}
\def\bfR{{\mathbf R}}
\def\bfS{{\mathbf S}}
\def\bfT{{\mathbf T}}
\def\bfU{{\mathbf U}}
\def\bfV{{\mathbf V}}
\def\bfW{{\mathbf W}}
\def\bfX{{\mathbf X}}
\def\bfY{{\mathbf Y}}
\def\bfZ{{\mathbf Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%bold symbols

\def\alphabf{\hbox{\boldmath$\alpha$\unboldmath}}
\def\betabf{\hbox{\boldmath$\beta$\unboldmath}}
\def\gammabf{\hbox{\boldmath$\gamma$\unboldmath}}
\def\deltabf{\hbox{\boldmath$\delta$\unboldmath}}
\def\epsilonbf{\hbox{\boldmath$\epsilon$\unboldmath}}
\def\zetabf{\hbox{\boldmath$\zeta$\unboldmath}}
\def\etabf{\hbox{\boldmath$\eta$\unboldmath}}
\def\iotabf{\hbox{\boldmath$\iota$\unboldmath}}
\def\kappabf{\hbox{\boldmath$\kappa$\unboldmath}}
\def\lambdabf{\hbox{\boldmath$\lambda$\unboldmath}}
\def\mubf{\hbox{\boldmath$\mu$\unboldmath}}
\def\nubf{\hbox{\boldmath$\nu$\unboldmath}}
\def\xibf{\hbox{\boldmath$\xi$\unboldmath}}
\def\pibf{\hbox{\boldmath$\pi$\unboldmath}}
\def\rhobf{\hbox{\boldmath$\rho$\unboldmath}}
\def\sigmabf{\hbox{\boldmath$\sigma$\unboldmath}}
\def\taubf{\hbox{\boldmath$\tau$\unboldmath}}
\def\upsilonbf{\hbox{\boldmath$\upsilon$\unboldmath}}
\def\phibf{\hbox{\boldmath$\phi$\unboldmath}}
\def\chibf{\hbox{\boldmath$\chi$\unboldmath}}
\def\psibf{\hbox{\boldmath$\psi$\unboldmath}}
\def\omegabf{\hbox{\boldmath$\omega$\unboldmath}}
\def\Sigmabf{\hbox{$\bf \Sigma$}}
\def\Upsilonbf{\hbox{$\bf \Upsilon$}}
%\def\Phibf{\hbox{$\bf \Phi$}}
%\def\Psibf{\hbox{$\bf \Psi$}}
\def\Omegabf{\hbox{$\bf \Omega$}}
\def\Deltabf{\hbox{$\bf \Delta$}}
\def\Gammabf{\hbox{$\bf \Gamma$}}
\def\Thetabf{\hbox{$\bf \Theta$}}
\def\Lambdabf{\mbox{$ \bf \Lambda $}}
\def\Xibf{\hbox{\bf$\Xi$}}
\def\Pibf{{\bf \Pi}}
%\def\thetabf{\hbox{\boldmath$\theta$\unboldmath}}
\def\thetabf{{\mbox{\boldmath$\theta$\unboldmath}}}
%\def\thetabf{\hbox{$\bf{\theta}$}}
\def\Upsilonbf{\hbox{\boldmath$\Upsilon$\unboldmath}}
\newcommand{\Phibf}{\mbox{${\bf \Phi}$}}
\newcommand{\Psibf}{\mbox{${\bf \Psi}$}}
\def\olambda{\mathfrak{o}(\lambda)}
\def\complex{\mathfrak{C}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Calligraphic
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%mathbb
\def\Abb{{\mathbb A}}
\def\BBb{{\mathbb B}}% different
\def\Cbb{{\mathbb C}}
\def\Dbb{{\mathbb D}}
\def\Ebb{{\mathbb E}}
\def\Fbb{{\mathbb F}}
\def\Gbb{{\mathbb G}}
\def\Hbb{{\mathbb H}}
\def\Ibb{{\mathbb I}}
\def\Jbb{{\mathbb J}}
\def\Kbb{{\mathbb K}}
\def\Lbb{{\mathbb L}}
\def\Mbb{{\mathbb M}}
\def\Nbb{{\mathbb N}}
\def\Obb{{\mathbb O}}
\def\Pbb{{\mathbb P}}
\def\Qbb{{\mathbb Q}}
\def\Rbb{{\mathbb R}}
\def\Sbb{{\mathbb S}}
\def\Tbb{{\mathbb T}}
\def\Ubb{{\mathbb U}}
\def\Vbb{{\mathbb V}}
\def\Wbb{{\mathbb W}}
\def\Xbb{{\mathbb X}}
\def\Ybb{{\mathbb Y}}
\def\Zbb{{\mathbb Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%command abbreviations
\newcommand{\bp}{\begin{psfrags}}
\newcommand{\ep}{\end{psfrags}}
\newcommand{\bl}{\begin{lemma}}
\newcommand{\el}{\end{lemma}}
\newcommand{\bt}{\begin{theorem}}
\newcommand{\et}{\end{theorem}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
%\newcommand{\bd}{\begin{definition}}
\newcommand{\ed}{\end{definition}}
\def\beq{\vskip .1cm \begin{equation}}
\def\eeq{\end{equation} \vskip .1cm \noindent}
\def\beqn{\vskip .1cm \begin{eqnarray}}
\def\eeqn{\end{eqnarray} \vskip .1cm \noindent}
\def\beqnn{\vskip .01cm \begin{eqnarray*}}
\def\eeqnn{\end{eqnarray*} \vskip .01cm \noindent}
\def\endproof{\hfill\blacksquare}
\def\defeq{:=}
\newcommand{\bim}{\begin{mylist}}
\newcommand{\eim}{\end{mylist}}
\def\bcase{\vskip .1cm \begin{numcases}}
\def\ecase{\end{numcases} \vskip .1cm \noindent}
\def\bsbcase{\vskip .1cm \begin{subnumcases}}
\def\esbcase{\end{subnumcases} \vskip .1cm \noindent}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%theorems

%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}
%\newtheorem{definition}{Definition}
%\newtheorem{problem}{Problem}
%\newtheorem{assumption}{A}
%\newtheorem{properties}{Properties}
%\newtheorem{conjecture}{Conjecture}
%\newtheorem{criterion}{Criterion}
%\newtheorem{proposition}{Proposition}
%\newtheorem{remark}{Remark}
%\newtheorem{notation}{Notation}
%\newtheorem{derivation}{Derivation}
%\newtheorem{proof}{Proof}
\newtheorem{claim}{Claim}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\matplottc}[1]{               % single matlab plot twocolumn
        \unitlength .45truein
        \begin{center}
        \begin{picture}(5,4.6)(1.05,.45)
        \special{psfile=#1.ps hscale=50 vscale=50}
        \end{picture}
        \end{center}
}
\newcommand{\matplotfp}[1]{               % single matlab plot fullpage
        \unitlength .45truein
        \begin{center}
        \begin{picture}(14,16)(.8,-1)
        \special{psfile=#1.ps hscale=100 vscale=100}
        \end{picture}
        \end{center}
}
\newcommand{\matplothp}[1]{               % single matlab plot halfpage
        \unitlength .45truein
        \begin{center}  \begin{picture}(14,7.5)(-1,.55)
        \special{psfile=#1.ps hscale=80 vscale=80}
        \end{picture}
        \end{center}
}
\newcommand{\matplothptop}[1]{               % single matlab plot halfpage
        \unitlength .45truein                % when figure is top of page
        \begin{center}  \begin{picture}(14,6.3)(-1,1.15)
        \special{psfile=#1.ps hscale=80 vscale=80}
        \end{picture}
        \end{center}
}
\newcommand{\matplotcc}[4]{             % two axis('square') plots side by side
        \vspace{2.8in}
        \special{psfile=#1.ps voffset=-10 hoffset=-22 vscale=52 hscale=52}
        \special{psfile=/user/xu/isl/matlab/psfiles/#2.ps voffset=-10 hoffset=213 vscale=52 hscale=52}
        \hspace*{\fill}\hspace*{0.35in}#3\hspace*{\fill}\hspace*{\fill}\hspace*{
0.35in}#4\hspace*{\fill} }
\newcommand{\matplottwo}[4]{             % two axis('normal') plots side by side
        \vspace{2.62in}
        \special{psfile=#1.ps voffset=-10 hoffset=-27 vscale=52 hscale=52}
        \special{psfile=#2.ps voffset=-10 hoffset=218 vscale=52 hscale=52}
        \vspace*{0.18in}
        \hspace*{\fill}\hspace*{-.05in}#3\hspace*{\fill}\hspace*{\fill}\hspace*{
0.65in}#4\hspace*{\fill} } %%
%% This is for making fancy paragraphs
%%
\def\psfancypar#1#2{\begingroup\def\par{\endgraf\endgroup\lineskiplimit=0pt}
               \setbox2=\hbox{\large\sc #2}
%              \showthe\lht2\showthe\baselineskip
               \newdimen\tmpht \tmpht \ht2 \advance\tmpht by \baselineskip
%              \showthe\tmpht
% Changed 10/2/89 rhr - t-bol -> Times-Bold for dvi2ps to dvips conversion
%              \font\hhuge=t-bol at \tmpht
               \font\hhuge=Times-Bold at \tmpht
               \setbox1=\hbox{{\hhuge #1}}
%              \showthe\ht1
               \count7=\tmpht \count8=\ht1
%  note that all this BS is necessary since TeX only does integer
%  divides and rounds all results
               \divide\count8 by 1000 \divide\count7 by \count8
%               \showthe\count7
               \tmpht=.001\tmpht\multiply\tmpht by \count7
%               \showthe\tmpht
%              \font\hhuge=t-bol at \tmpht
               \font\hhuge=Times-Bold at \tmpht
               \setbox1=\hbox{{\hhuge #1}}
               \noindent
                \hangindent1.05\wd1
               \hangafter=-2 {\hskip-\hangindent
               \lower1\ht1\hbox{\raise1.0\ht2\copy1}%
                \kern-0\wd1}\copy2\lineskiplimit=-1000pt}


\newenvironment{ap}{
\renewcommand{\thesection}{\mbox{Appendix }\Alph{section}}
\renewcommand{\thesubsection}{\Alph{section}.\arabic{subsection
}}
\renewcommand{\theequation}{\mbox{\Alph{section}.}\arabic{equation}}
}{
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\theequation}{\arabic{equation}}
}
%\setlength{\footnoterulewidth}{0.5pt}

%\setlength{\floatsep}{0.1cm}

%\setlength{\textfloatsep}{0.1cm}

%\setlength{\intextsep}{0.1cm}

%\setlength{\abovecaptionskip}{0.1cm}
%
%\setlength{\belowcaptionskip}{0.1cm}
%
%\setlength{\topsep}{0.1cm}
%
%\setlength{\partopsep}{0.1cm}
%
%\setlength{\itemsep}{0.1cm}
%
\setlength{\parindent}{0mm}
%
%\setlength{\dbltextfloatsep}{0.1cm}
%
%\setlength{\dblfloatsep}{0.1cm}
%
%\addtolength{\abovedisplayskip}{-1.5em}
%
%\addtolength{\belowdisplayskip}{-1.5em}
%
%\setlength{\arraycolsep}{0.1cm}

%\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern3pt
%        \vbox{\kern3pt#1\kern3pt}\kern3pt\vrule}\hrule}}
%\def\dag{{\cal y}}
%\def\reals{ { {\rm  I \kern-0.15em R }  } }
%\def\complex{ {\,{{\rm C} \kern-0.50em \raise0.20ex {  |}}\, }}


%
%\newtheorem{theorem}{Theorem}[chapter]
%\newtheorem{conjecture}{Conjecture}[chapter]
%\newtheorem{lemma}{Lemma}[chapter]
%\newtheorem{definition}{Definition}[chapter]
%\newtheorem{corollary}{Corollary}[chapter]


%\newcounter{remarknr}[chapter]
%\newenvironment{remark}{\vskip\baselineskip
%\stepcounter{remarknr}\noindent{\bf
%Remark~\theremarknr.}}{\ \hfill $\Box$ \vskip\baselineskip}
%\newcounter{examplenr}[chapter]
%\newenvironment{example}[1]{\vskip\baselineskip
%\stepcounter{examplenr}\noindent{{\bf
%Example~\thechapter.\theexamplenr}\hskip .8em #1\\}}{\ \hfill $\Box$
%\vskip\baselineskip}




%\newcommand{\x}{\mbox{${\bf x}(t)$}}
%\newcommand{\s}{\mbox{${\bf s}(t)$}}
%\newcommand{\n}{\mbox{${\bf n}(t)$}}
%\newcommand{\jj}{\mbox{${\bf j}(t)$}}
%\newcommand{\R}{\mbox{$\hat {\bf R}_{N}$}}
%\newcommand{\Rhat}{\mbox{$\hat {\bf R}$}}
%\newcommand{\A}{\mbox{${\cal A}$}}
%\newcommand{\Ad}{\mbox{${\cal A}^d$}}
%\newcommand{\D}{\mbox{${\cal D}$}}
%\newcommand{\M}{\mbox{{\bf M}}}
%\newcommand{\Tr}{\mbox{Tr}}
%\newcommand{\pbox}{\hfill $\Box$}
%\newcommand{\blankline}{\vskip\baselineskip\noindent}
%\def\Rxx{\Rbf_{\ssstyle X\kern-.1em X}}
%\def\rxx{\hbox{$\Rxx$}}
%\def\ryy{\hbox{$\Rbf_{\ssstyle YY}$}}
%\def\rxy{\hbox{$\Rbf_{\ssstyle XY}$}}\def\ryx{\hbox{$\Rbf_{\ssstyle YX}$}}
%\def\rxyT{\hbox{$\Rbf_{\ssstyle XY}^*$}}\def\ryxT{\hbox{$\Rbf_{\ssstyle YX}^*$}}
%\def\Rss{\Rbf_{\ssstyle SS}}
%\def\rss{\mbox{$\Rss$}}
%\def\Rnn{\Rbf_{\ssstyle NN}}
%\def\rnn{\hbox{$\Rnn$}}
%\def\rxxinv{\hbox{$\Rbf^{-1}_{\ssstyle XX}$}}
%\def\Rssinv{\Rbf^{-1}_{\ssstyle SS}}
%\def\rssinv{\hbox{$\Rssinv$}}
%\def\rzzinv{\Rbf^{-1}_{\ssstyle ZZ}}\let\rzzi=\rzzinv
%\def\hatrxx{\widehat{\Rbf}_{\ssstyle XX}}
%\def\hatrzz{\widehat{\Rbf}_{\ssstyle ZZ}}
%\def\hatrss{\widehat{\Rbf}_{\ssstyle SS}}
%\def\phstar{{\phantom{*}}}
%\let\rzzhat=\hatrzz \let\rxxhat=\hatrxx \let\Rxxhat=\rxxhat
%\let\ssstyle=\scriptscriptstyle
%\let\rsshat=\hatrss


% I add the following!
%\def\eqorneq{=\!\!\!\! ? \,\,}
%\def\ltornlt{? \!\!\!\!\! <}
%\def\sN{{\ssstyle N}}
%\def\sM{{\ssstyle M}}
%\def\sF{{\ssstyle F}}
%\def\sT{{\ssstyle T}}
%\def\sH{{\ssstyle H}}
%\def\sK{{\ssstyle K}}
%\def\sL{{\ssstyle L}}
%\def\sQ{{\ssstyle Q}}
%\def\sV{{\ssstyle V}}
%\def\cross{\!  \times  \!}
%\def\alphat{\alpha^{(t)}}
%\def\alphab{\alpha^{(b)}}
%\def\betat{\beta^{(t)}}
%\def\betab{\beta^{(b)}}
%\def\ATbf{{\bf A_\sT}}
%\def\AHbf{{\bf A_\sH}}
%\def\sspan{\mbox{\it span}}



\def\Kout{\setbox1=\hbox{\Huge\bf K}\hbox to
1.05\wd1{\hspace{.05\wd1}\special{
"/Times-BoldItalic findfont 25 scalefont setfont
/prKzip
{0 0 moveto (K) show} def
/dozip
{gsave
  /xp 0 def
  .08 -.04 0
  {
   setgray
  prKzip
%  /xp xp dx add def xp -.7 translate %for
  -.7 .4 translate} for
  1 setgray prKzip
  0 0 moveto
  0 setgray
  .5 setlinewidth
  (K) true charpath  stroke
 grestore
} def
dozip}}}
\def\Sout{\setbox1=\hbox{\Huge\bf S}\hbox to 1.05\wd1{\hspace{.05\wd1}\special{"
/Times-BoldItalic findfont 25 scalefont setfont
/prSzip
{0 0 moveto (S) show} def
/dozip
{gsave
  /xp 0 def
  .08 -.04 0
  {
   setgray
  prSzip
%  /xp xp dx add def xp -.7 translate %for
  -.7 .4 translate} for
  1 setgray prSzip
  0 0 moveto
  0 setgray
  .5 setlinewidth
  (S) true charpath  stroke
 grestore
} def
dozip}}}

%\newcommand{\thhat}{\mbox{${\hat{\thetabf}}_N$}}
%\newcommand{\thbar}{\mbox{${\bar{\thetabf}}_N$}}
%\newcommand{\etahat}{\mbox{${\hat{\etabf}}$}}
%\newcommand{\etabf}{\mbox{${\bf\eta}$}}
%\newcommand{\e}{\mbox{${\bf e}_k$}}
%\newcommand{\ehat}{\mbox{$\hat{\bf e}_k$}}
%\newcommand{\EWE}{\mbox{${\bf E}_s^{}{\bf WE}_s^*$}}
%\newcommand{\DPD}{\mbox{$\Dbf^*\Pbf_{\bf A}^{\perp} \Dbf$}}
%\newcommand{\EWEhat}{\mbox{$\hat{\bf E}_s^{}{\bf W}\hat{\bf E}_s^*$}}
%\newcommand{\E}{\mbox{{\rm E}}}
%\newcommand{\Efs}{\mbox{${\bf E}_s^{}$}}
%\newcommand{\En}{\mbox{${\bf E}_n^{}$}}
%\newcommand{\Eshat}{\mbox{$\hat{\bf E}_s^{}$}}
%\newcommand{\Lshat}{\mbox{$\hat {\bf \Lambda}_s^{}$}}
%\newcommand{\Ls}{\mbox{$ {\bf \Lambda}_s^{}$}}
%\newcommand{\Ln}{\mbox{$ {\bf \Lambda}_n^{}$}}
%\newcommand{\Ltilde}{\mbox{$\widetilde {\bf \Lambda}$}}
%\newcommand{\Enhat}{\mbox{$\hat{\bf E}_n^{}$}}
%\newcommand{\Lnhat}{\mbox{$\hat {\bf \Lambda}_n^{}$}}
%\newcommand{\Ai}{\mbox{$ ({\bf A}^*{\bf A})^{-1} $}}
%\newcommand{\abf}{\mbox{${\bf a}$}}


%Define affiliation at footnote
% Make \small be smaller (8 pt)
%\def\small{\@setsize\small{9pt}\viiipt\@viiipt\let\@listi\@listI}


%%%%% notation %%%%%
%Anima added
\DeclareMathOperator{\Map}{Map}
\def\convp{{\stackrel{\mathrm{P}}{\to}}}

\def\qed{\hfill\hbox{${\vcenter{\vbox{
    \hrule height 0.4pt\hbox{\vrule width 0.4pt height 6pt
    \kern5pt\vrule width 0.4pt}\hrule height 0.4pt}}}$}}

\def\Depth{\delta}
\def\Hops{{\mbox{Hops}}}

% Variables
\newcommand{\wloc}{W} % graph
\newcommand{\loc}{L}
\newcommand{\wpre}{c}
%\newcommand{\neighbors}{\mathcal{N}}
%\newcommand{\clneighbors}{\mathcal{N}^{CL}}
%\newcommand{\nodes}{\mathcal{V} \cup \mathcal{H}}
%\newcommand{\onodes}{\mathcal{V}}
%\newcommand{\hnodes}{\mathcal{H}}
%\newcommand{\inodes}{\mathcal{I}}

\newcommand{\rc}{r}
\newcommand{\idtree}{\mathcal{T}_I}
\newcommand{\tree}{T}
\newcommand{\cltree}{\tree^{CL}}
\newcommand{\subtree}{\mathcal{S}}

% Vincent added
\newcommand{\calV}{\mathcal{V}}
\newcommand{\WW}{W}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hd}{\hat{d}}
\newcommand{\hPhi}{\hat{\Phi}}
\newcommand{\hbd}{\hat{\bd}}
\newcommand{\hmu}{\hat{\mu}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\hT}{\hat{T}}
\newcommand{\ML}{\mathrm{ML}}
\newcommand{\Sg}{\mathrm{Sg}}
\newcommand{\calO}{\mathcal{O}}
%\newcommand{\Path}{\mathrm{Path}}
\newcommand{\diam}{\mathrm{diam}}
\newcommand{\MST}{\mathrm{MST}}
\newcommand{\Leaf}{\mathrm{Leaf}}
\newcommand{\brho}{\bm{\rho}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bDelta}{\bm{\Delta}}
%\newcommand{\nbd}{\mathrm{nbd}}
\newcommand{\bR}{\mathbb{R}}

%\DeclareMathOperator*{\argmax}{argmax}
%\DeclareMathOperator*{\argmin}{argmin}

\newtheorem{THEO}{\bf Theorem}
\newtheorem{CORL}[THEO]{\bf Corollary}
\newtheorem{LEMM}[THEO]{\bf Lemma}
\newtheorem{REMA}{\bf Remark}
\newtheorem{DEFI}{\bf Definition}
\newtheorem{CLAIM}{\bf Claim}
\newtheorem{PROP}[THEO]{\bf Proposition}
\newtheorem{PROOF}{\bf Proof}
\newtheorem{EXAMPLE}{\bf Example}
\newtheorem{FACT}{\bf Fact}


\newcommand{\mathdef}{:=}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\mat}{mat}
\DeclareMathOperator{\Rank}{Rank}

\def\nbd{\mathcal{N}}
\def\Path{{\mathrm{Path}}}

\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\polylog}{polylog}
\def\veps{\varepsilon}
%\newcommand{\calX}{\mathcal{X}}
%\newcommand{\qed}{\hfill \ensuremath{\Box}}
%\newcommand{\bX}{\mathbf{X}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\ba}{\mathbf{a}}
%\newcommand{\calG}{\mathcal{G}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calN}{\mathcal{N}}
%\renewcommand{\calE}{E}
\newcommand{\hcalU}{\widehat{\mathcal{U}}}
%\renewcommand{\calV}{V}
%\newcommand{\calB}{\mathcal{B}}
%\newcommand{\calT}{\mathcal{T}}
%\newcommand{\calA}{\mathcal{A}}
%\newcommand{\calD}{\mathcal{D}}
%\newcommand{\bx}{\mathbf{x}}
%\newcommand{\0}{\mathbf{0}}
%\newcommand{\bR}{\mathbb{R}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calY}{\mathcal{Y}}
%\newcommand{\calH}{\mathcal{H}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bL}{\mathbf{L}}
%\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bmeta}{\bm{\eta}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bxi}{\bm{\xi}}
%\newcommand{\bK}{\mathbf{K}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
%\newcommand{\hp}{\widehat{p}}
%\newcommand{\argmin}{\operatornamewithlimits{argmin}}
%\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\hP}{\widehat{P}}
\newcommand{\hrho}{\widehat{\rho}}
\newcommand{\hPML}{{P}_{{\text{\tiny ML}}}}
\newcommand{\hI}{\widehat{I}}
\newcommand{\hQ}{\widehat{Q}}
\newcommand{\PML}{P_{\mathrm{ML}}}
\newcommand{\hTML}{{T}_{\text{\tiny ML}}}
%\newcommand{\Path}{\mathrm{Path}}
\newcommand{\tilp}{\widetilde{p}}
\newcommand{\tilJ}{\widetilde{J}}
\newcommand{\tilP}{\widetilde{P}}
\newcommand{\tilQ}{\widetilde{Q}}
\newcommand{\tilK}{\widetilde{K}}
\newcommand{\beps}{\bm{\epsilon}}
\newcommand{\var}{\mathrm{Var}}
%\newcommand{\etal}{et al.\ }
\newcommand{\hcalE}{{\calE}_{{\text{\tiny ML}}}}

\newcommand{\boxedeqn}[1]{%
  \[\fbox{%
      \addtolength{\linewidth}{-2\fboxsep}%
      \addtolength{\linewidth}{-2\fboxrule}%
      \begin{minipage}{\linewidth}%
      \begin{equation}#1\end{equation}%
      \end{minipage}%
    }\]%
}

\newtheorem*{theo}{Theorem}
\newtheorem*{proposition}{Proposition} 

\renewcommand{\thefootnote}{}





\newcommand{\fhcomment}{\textcolor[rgb]{1,0,0}{FH: }\textcolor[rgb]{1,0,0}} 
\renewcommand{\thefootnote}{}
\DeclareMathOperator{\Pairs}{Pairs}
\newcommand{\llvert}{\left\vert\vphantom{\frac{1}{1}}\right.}
\newcommand{\Pvalue}{\mathsf{P_{\text{val}}}}
\newcommand{\HRule}{\rule{\linewidth}{0.1mm}}
\def\nbd{\mathcal{N}}
\def\Path{{\mathrm{Path}}}

\def\veps{\varepsilon}
\newcommand{\Toep}{\mathsf{Cir}}
\DeclareMathOperator{\opt}{opt}
\newcommand{\DFT}{\mathsf{FFT}}
\newcommand*{\hermconj}{^{\mathsf{H}}}
\newcommand\supp{\operatorname{supp}}
\renewcommand{\thefootnote}{}
\def\veps{\varepsilon}
\DeclareMathOperator{\Cum}{C_3}
\DeclareMathOperator{\myblock}{blk}
\def\nbd{\mathcal{N}}
\def\Path{{\mathrm{Path}}}
\newcommand{\thetastar}{\ensuremath{\theta^*}}
\newcommand{\Astar}{\ensuremath{A^*}}
\newcommand{\Xstar}{\ensuremath{X^*}}
\newcommand{\iprod}[2]{\langle #1, #2 \rangle}
\newcommand{\Aiter}[1][t]{\ensuremath{A(#1)}}
\newcommand{\Aiteri}[1][t]{\ensuremath{A_i(#1)}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\order}{\ensuremath{\mathcal{O}}}
\newcommand{\Xiter}[1][t]{\ensuremath{X(#1)}}
\newtheorem{assumption}{Assumption}
\newtheorem{goal}{Goal}
\newcommand{\Nb}{\text{nbd}}
\DeclareMathOperator{\Adj}{\mathcal{N}}
\def\ourframework{{$\textsf{ConvDic}$$+$$\textsf{DeconvDec}$ }}



% Definitions in paper
\newcommand*{\mytensor}[1]{\bm{\mathcal{#1}}}
\newcommand*{\mymatrix}[1]{\bm{#1}}
\newcommand*{\myvector}[1]{\bm{#1}}
\newcommand*{\noise}[1]{\widehat{#1}}
\newcommand*{\mm}{\mymatrix}
\newcommand*{\mv}{\myvector}
\newcommand{\mt}{\mytensor}
\newcommand*{\mmCols}[2]{\mm{#1}_{[#2]}}
% names
\newcommand{\ourmod}{{GIM}\xspace}
\newcommand{\ourmodfull}{{Greedy Inference Model}\xspace}
\newcommand{\dmname}{{dynamic matrix}\xspace}
\newcommand{\dmnames}{{dynamic matrices}\xspace}
\newcommand{\avgrew}{{AvgReward}\xspace}
\newcommand{\pavgrew}{{PostAvgReward}\xspace}
\newcommand{\numepi}{{TotalEps}\xspace}
\newcommand{\walkname}{{$\beta$-curious walking}\xspace}

% about dynamic matrices
\newcommand{\states}{\mathcal{S}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\dmat}{\mymatrix{M}}
\newcommand{\dmats}{M}
\newcommand{\admat}{\mymatrix{\hat{M}}}
\newcommand{\rdmat}{\mymatrix{\widetilde{M}}}
\newcommand{\rdmats}{\widetilde{M}}
\newcommand{\dmatset}{\{\mymatrix{M}^k\}_{k=1}^{S+1}}
\newcommand{\admatset}{\{\mymatrix{\hat{M}}^k\}_{k=1}^{S+1}}
\newcommand{\rdmatset}{\{\mymatrix{\widetilde{M}}^k\}_{k=1}^{S+1}}
\newcommand{\krange}{1,2,\cdots,S+1}


% about mask
\newcommand{\mask}{\mymatrix{P}^\mathcal{K}}
\newcommand{\masks}{P^\mathcal{K}}
\newcommand{\kset}{\mathcal{K}}
\newcommand{\nkset}{\bar{\mathcal{K}}}

% about noise
\newcommand{\noiset}{\mytensor{Z}}
\newcommand{\noisem}{\mymatrix{Z}}
\newcommand{\noises}{Z}

\newcommand{\fraction}{\rho}

\newcommand{\minsa}{M_{in}}
\newcommand{\maxsa}{M_{ax}}

\DeclareMathOperator*{\minimize}{\text{minimize}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


==> include/talks/supp_packages.tex <==
\usepackage[mathscr]{eucal}
\usepackage{bm,verbatim,pifont,color,amssymb,amsfonts,amsmath,graphicx,epsf,psfrag,ifpdf,xmpmulti,cases,hyperref}
% \usepackage{slashbox}
\usepackage[english]{babel}
\usepackage[fleqn,tbtags]{mathtools}
\usepackage{amsmath}
\usepackage[attachfiles]{media9}
\usepackage{mathtools}
\usepackage{media9}
%\usepackage{multimedia}
\usepackage{pgfpages}
\usepackage{siunitx}
\usepackage{tablefootnote}
\usepackage{xspace}

\usepackage{tikz}
\usetikzlibrary{fit}
\usetikzlibrary{calc,shapes}
\usetikzlibrary{decorations.pathmorphing} % noisy shapes
\usetikzlibrary{fit}					% fitting shapes to coordinates
\usetikzlibrary{backgrounds}	% drawing the background after the foreground
%pgfplots
\usepackage[utf8]{inputenc}
% \usepackage{fontspec}  % optional
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{dateplot}

\usepackage{tcolorbox}
\usepackage{pgfpages}
%\usecolortheme{seagull}
%\definecolor{uofsgreen}{rgb}{.125,.5,.25}
%\usecolortheme[named=orange]{structure}
%\usecolortheme{rose}
%\usecolortheme{lily}
%\usecolortheme{rose}
%\usecolortheme{dolphin}
%\usecolortheme[rgb={0,0.17,0.45}]{structure}


%\usecolortheme{default}
%\usepackage[english]{babel}
% or whatever

%\usepackage[latin1]{inputenc}
% or whatever

\usepackage{colortbl}
%\usepackage{times}
%\usepackage[T1]{fontenc}
\usepackage{multimedia}
%\usepackage{latexsym, amssymb, amsmath}
%\setcounter{tocdepth}{3}
%\usepackage{graphicx}
%\usepackage{url}
%\usepackage{color}
%\usepackage{bm}
\usepackage{multirow}

%\usecolortheme{whale}
% \usecolortheme{beetle}
%\usecolortheme[named=seahorse]{structure}
%seahorse% seagull %beaver  albatross % lily %albatross %beetle %whale %crane
%\usecolortheme{default}
%\usepackage[english]{babel}
% or whatever
%
%\usepackage[latin1]{inputenc}
% or whatever
%
%\usepackage[lined, algonl, boxed]{algorithm2e}

\usepackage{algorithmic}
\usepackage{algorithm}
%\usepackage{subfigure}
%\usepackage{times}
%\usepackage[T1]{fontenc}
%\usepackage{hyperref}
%\usepackage{multimedia}
%\usepackage{latexsym, amssymb, amsmath}
%\setcounter{tocdepth}{3}
%\usepackage{graphicx}
%\usepackage{url}
%\usepackage{color}
%\usepackage{bm}

==> proofs/main_thm.tex <==
%!TEX root = ../0_neurips19_tensor_rl_main.tex
\begin{proof} (of Theorem~\ref{thm:main}) 
By replacing the known threshold $m$ in Lemma~\ref{lem:sc_m} with the result of Section~\ref{sec:set_m}, 
% as well as setting the failure probability of exploration and satisfying Equation~\ref{eq:m_cond_k} and \ref{eq:m_cond_all} to be all $\delta/3$, we can derive to the theorem.
as well as setting the failure probability of exploration and satisfying Condition~\ref{cond:m} to be both $\delta/2$, we can derive to the theorem.


















\end{proof}
